Learning Predictive Visuomotor Coordination

Understanding and predicting human visuomotor coordination is crucial for applications in robotics, human-computer interaction, and assistive technologies. This work introduces a forecasting-based task for visuomotor modeling, where the goal is to predict head pose, gaze, and upper-body motion from egocentric visual and kinematic observations. We propose a \textit{Visuomotor Coordination Representation} (VCR) that learns structured temporal dependencies across these multimodal signals. We extend a diffusion-based motion modeling framework that integrates egocentric vision and kinematic sequences, enabling temporally coherent and accurate visuomotor predictions. Our approach is evaluated on the large-scale EgoExo4D dataset, demonstrating strong generalization across diverse real-world activities. Our results highlight the importance of multimodal integration in understanding visuomotor coordination, contributing to research in visuomotor learning and human behavior modeling. Project Page: https://vjwq.github.io/VCR/.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> sec/0_abstract.tex <==
% \vspace{6pt}
\begin{abstract}
% Understanding how head motion, gaze behavior, and upper-body dynamics co-evolve is essential for applications in robotics, AR, and human–computer interaction. In this paper, we propose a task of predictive visuomotor coordination, where we aim to forecast head pose, gaze target, and upper-body motion from past egocentric visual and kinematic observations. To capture these coupled signals, we introduce a unified Visuomotor Coordination Representation (VCR), which organizes head, gaze, and arm cues into a coherent visuomotor state. Building on this representation, we develop a multimodal diffusion-based model that fuses egocentric visual context with structured visuomotor cues for accurate prediction. Experiments on the large-scale EgoExo4D dataset show consistent improvements across diverse real-world activities, highlighting the importance of joint head–gaze–arm modeling for visuomotor forecasting. 
\let\thefootnote\relax\footnotetext{$\dagger$ Equal advising.}
% Our results demonstrate that forecasting the coupled future trajectories of head, gaze, and upper-body motion provides a precise model of visuomotor coordination in natural task settings. 
Understanding the joint evolution of head motion, gaze behavior, and upper-body dynamics is essential for applications in robotics, AR, and human–computer interaction. In this paper, we propose a predictive visuomotor coordination task that forecasts head pose, 3D gaze endpoints, and upper-body motion from egocentric visual and kinematic observations. To model these signals jointly, we introduce a Visuomotor Coordination Representation (VCR), which organizes them into a unified state. Building on this representation, we develop a multimodal diffusion model that fuses egocentric visual context with structured kinematic cues. Experiments on EgoExo4D demonstrate consistent improvements across diverse real-world activities. Our results highlight the importance of modeling coupled visuomotor dynamics for accurate forecasting. Project page: \href{http://vjwq.github.io/VCR}{http://vjwq.github.io/VCR}.
% Understanding and predicting human visuomotor coordination is crucial for applications in robotics, human-computer interaction, and assistive technologies. This work introduces a forecasting-based task for visuomotor modeling, where the goal is to predict head pose, gaze, and upper-body motion from egocentric visual and kinematic observations. We propose a \textit{Visuomotor Coordination Representation} (VCR) that learns structured temporal dependencies across these multimodal signals. We extend a diffusion-based motion modeling framework that integrates egocentric vision and kinematic sequences, enabling temporally coherent and accurate visuomotor predictions. Our approach is evaluated on the large-scale EgoExo4D dataset, demonstrating strong generalization across diverse real-world activities. Our results highlight the importance of multimodal integration in understanding visuomotor coordination, contributing to research in visuomotor learning and human behavior modeling. 

\end{abstract}

==> sec/1_intro.tex <==
% \vspace{-12pt}
\section{Introduction}
\label{sec:intro}
Human visuomotor coordination is essential to action planning and execution, integrating first-person visual perception, head orientation, and proprioceptive control to produce fluid, goal-directed movements~\cite{zago2009visuo}. Rather than functioning as a purely reactive system, it operates \textbf{\textit{predictively}}~\cite{wolpert2001motor,shadmehr2010error,avraham2019effects}, using recent sensory input to anticipate upcoming demands and to compensate for inherent sensory and neural delays~\cite{nijhawan2009compensating}. 
% This predictive nature manifests in the coupled behavior of head pose, gaze allocation, and upper-body motion during everyday activities.
% Predicting how a person will move in the next few seconds is a core capability for egocentric vision, with applications in augmented reality assistance and human–robot interaction. 
% In order for an AI assistant in a pair of smart eyeglasses to be helpful, it should be able to anticipate what a person might be trying to do and provide advice or interventions before a problem occurs.
% To support a camera wearer in real time, an AI system must anticipate how the head will turn, where the gaze will shift, and how the upper body will respond to task cues. 
% Coupled behavior of head orientation, gaze allocation, and upper-body motion is fundamental in human daily activities. 
% We refer to this coupled behavior of head orientation, 3D gaze allocation, and upper-body motion as \textit{Visuomotor Coordination}, and study it through the task of forecasting its future states from past observations. 

% Despite the anticipatory nature of visuomotor behavior, existing computational models 
Prior work in anticipatory egocentric vision typically focuses on forecasting individual signals, rarely capturing their full multimodal structure. Examples include saliency-based 2D gaze distributions~\cite{lai2022eye,lai2024listen}, hand trajectories~\cite{jia2022generative,liu2022joint}, and upper-body pose~\cite{escobar2025egocast,chen2025egoagent}. However, these modalities are typically modeled in isolation. As a result, they do not capture 3D gaze endpoints or the head–gaze–arm coupling required for visuomotor coordination.
% Examples include saliency-based 2D gaze distributions~\cite{lai2022eye,lai2024listen}, hand trajectories~\cite{jia2022generative,liu2022joint}, or upper-body pose~\cite{escobar2025egocast,chen2025egoagent}, but these modalities are modeled in isolation and do not yield the 3D gaze endpoints or head–gaze–arm coupling required for visuomotor coordination. 
Related efforts in robotics focus on goal inference and imitation learning~\cite{Aronson2021,Saran2018,finn2017one,lynch2019learning,zeng2020transporter}, yet they typically rely on task-specific demonstrations and do not model the natural coordination between head, gaze, and upper-body motion. Bridging the gap between egocentric perception and coordinated human motion therefore remains an open challenge. Notably, explicit forecasting of 3D gaze endpoints has received limited attention, despite its central role in visuomotor behavior.
% Psychological studies show that visuomotor coordination is predictive, relying on visual memory to plan actions across several seconds\cite{hayhoe2003visual}. Modeling these anticipatory mechanisms can benefit downstreaming tasks for robotics, AR or VR, and human–computer interaction, where rapid inference of user intent is essential. Prior research in egocentric vision has made progress by forecasting individual signals such as saliency-based 2D gaze distributions\cite{lai2022eye,li2023ego}, hand trajectories\cite{jia2022generative,liu2022joint}, or body pose\cite{escobar2025egocast,chen2025egoagent}, but each modality is modeled independently and does not provide the geometric 3D gaze endpoints necessary for visuomotor coordination. Beyond egocentric vision, visuomotor prediction has also been explored in robotics to support manipulation and assistive tasks\cite{Aronson2021,Saran2018}. Learning from human demonstrations\cite{finn2017one,lynch2019learning,zeng2020transporter} enables robots to generalize across diverse actions, yet these approaches typically rely on task-specific datasets and do not model full-body visuomotor coordination in natural settings. Bridging the gap between egocentric perception and full-body visuomotor learning therefore remains an open challenge. To our knowledge, explicit forecasting of 3D gaze endpoints has not been largely explored, despite their central role in visuomotor coordination.

This is a fundamental limitation because natural visuomotor behavior is coordinated. Head orientation stabilizes visual perception, gaze shifts reveal upcoming goals, and arm movements unfold relative to the head–gaze reference frame. Methods that operate on isolated signals cannot explicitly capture this coupled structure, even when conditioning on egocentric video. Consequently, existing forecasting formulations cannot model how attention, viewpoint, and action evolve together in natural activities.

A major reason for this gap is the lack of datasets that jointly capture synchronized egocentric video, 3D head pose, 3D gaze, and upper-body motion. EgoExo4D~\cite{grauman2024ego} provides this combination through accurate SLAM-based head pose, 3D gaze endpoints, and aligned exocentric body motion, enabling large-scale analysis of human visuomotor behavior.

Building on this data foundation, we formulate a unified forecasting task that predicts the future evolution of head pose, 3D gaze endpoints, and upper-body motion from past egocentric visual and kinematic observations. This requires modeling temporal dependencies across signals that operate at different semantic levels, where gaze reflects intention, head orientation links perception to action, and upper-body motion encodes execution.

To address this challenge, we introduce a structured Visuomotor Coordination Representation and a multimodal diffusion model that fuses egocentric visual context with head, gaze, and upper-body cues. The architecture organizes kinematic signals into complementary paths that reflect the natural hierarchy of the visuomotor system and uses egocentric frames to provide task-level context. A canonicalization step enforces spatial and temporal consistency, allowing the model to learn relative motion patterns independent of global movement.

We evaluate our approach on EgoExo4D and show consistent improvements in predicting head pose, gaze position, and upper-body trajectories across diverse activities. These results demonstrate the importance of modeling head, gaze, and arm dynamics as a coordinated process. By treating human movement as a unified visuomotor system, our framework advances egocentric forecasting and provides foundations for future work in human–AI interaction, AR assistance, and robot imitation learning.
Our contributions are summarized as follows: 
\begin{itemize}
    \item We define the first unified visuomotor forecasting task that jointly predicts future head pose, gaze endpoint and upper-body motion from past egocentric visual and kinematic inputs.
    % \item We formulate a forecasting-based task for human visuomotor modeling, integrating head pose, gaze direction, fixation, and upper-body motion to capture temporal dependencies.
    \item We design a structured multimodal diffusion framework with separate head-gaze and head-gaze-arm pathways fused with visual context, providing conditioning that preserves cross-modal visuomotor relations. 
    % \item We extend a diffusion-based framework that integrates egocentric vision and kinematic sequences, leveraging multimodal fusion to enhance temporal coherence and prediction accuracy.  
    \item We conduct thorough evaluations on the EgoExo4D dataset, demonstrating consistently strong performance across diverse real-world activities.  
    \item We provide detailed analyses and ablations that reveal concrete dependencies among head motion, gaze behavior and upper-body dynamics in predictive coordination.
    % \item Our analysis includes extensive quantitative and qualitative evaluations, with a comprehensive ablation study assessing the impact of each multimodal component on accuracy.  
\end{itemize}


==> sec/1_intro_old.tex <==
% {\color{blue}\section{Introduction}}
\section{Introduction}
\label{sec:intro}
% Analyzing egocentric video to anticipate what the camera wearer will do next is a central problem in egocentric vision with applications in augmented reality (AR) and robotics. For AI assistants embedded in smart glasses to be useful, they must anticipate what a person is trying to do and offer guidance or intervention before errors occur. Prior work has explored forecasting individual signals such as ego-motion, gaze, and hand trajectories from egocentric video \cite{jia2022generative, lai2022eye, li2023ego}. However, these approaches typically model each modality in isolation and do not account for the tight temporal coupling among head orientation, gaze allocation, and upper-body movement. A key gap is the lack of models that capture the visuomotor control processes underlying natural goal-directed behavior.

% Psychological research highlights the predictive nature of visuomotor coordination. Hayhoe et al. \cite{hayhoe2003visual} showed that during natural tasks such as sandwich preparation, people use information from previous fixations to guide gaze shifts and coordinate hand movements several seconds into the future. Such predictive visuomotor behavior enables smooth interaction with the environment and suggests that jointly modeling these signals can support more effective anticipation in AR, VR, and human-robot interaction.

% Visuomotor prediction has also been studied in robotics to improve manipulation and assistive behaviors. Learning from human demonstrations \cite{finn2017one, lynch2019learning, zeng2020transporter} has enabled generalization across diverse tasks, yet these methods often rely on task-specific datasets and do not model full-body visuomotor coordination in natural settings. Connecting egocentric visual perception with three-dimensional human visuomotor forecasting therefore remains an open challenge.

% In this work, we address this challenge by formulating a unified visuomotor forecasting task that jointly predicts future head pose, gaze target, and upper-body motion in 3D from past egocentric visual and kinematic observations. Our approach uses a structured multimodal diffusion framework that integrates visual context with separate head-gaze and head-gaze-arm kinematic pathways, enabling the model to learn consistent temporal patterns across these complementary signals.

% Recent large-scale datasets such as EgoExo4D \cite{grauman2024ego} and Nymeria \cite{ma2024nymeria} provide synchronized 3D gaze, head pose, and body motion in diverse daily activities, making it possible to quantitatively study visuomotor forecasting. We evaluate our approach on EgoExo4D and additionally test cross-dataset generalization on the Nymeria egocentric motion dataset. Our results show that jointly modeling head, gaze, and upper-body cues leads to more coherent future predictions and offers new insights into the temporal structure of human visuomotor coordination.

Analyzing egocentric video to predict what the camera-wearer is going to do next is an important task in egocentric vision with applications in Augmented Reality (AR) and robotics. In order for an AI assistant in a pair of smart eyeglasses to be helpful, it should be able to anticipate what a person might be trying to do and provide advice or interventions \emph{before} a problem occurs. As a result, previous works have developed deep learning models to forecast ego-motion, gaze, and hand trajectories from egocentric videos \cite{jia2022generative,lai2022eye,liu2022joint}. However, most prior methods focus on isolated modality signals (e.g., only gaze or hand motion) and fail to model their multimodal interdependencies. A key missing element in these prior works is a detailed consideration of the visumotor control system which underlies all goal-directed human movement. 

Psychological research underscores the predictive nature of visuomotor coordination, particularly in how visual memory informs motor planning. Hayhoe et al. \cite{hayhoe2003visual} observed that during natural tasks like making a sandwich, individuals rely on visual information from previous fixations to plan and coordinate movements over the course of several seconds. This reliance on stored visual memory allows humans to anticipate object locations and properties, ensuring seamless interaction with the environment. We hypothesize that understanding and modeling these predictive visuomotor behaviors can provide more effective forecasting capabilities for robotics, VR/AR, and human-computer interaction, where anticipating human movement can enhance real-time decision-making and system adaptability.

Beyond egocentric vision, visuomotor prediction has also been explored in robotics to enhance manipulation and assistive tasks. Learning from human demonstrations \cite{finn2017one, lynch2019learning, zeng2020transporter} has enabled robots to generalize across diverse actions. However, these methods often rely on task-specific datasets and do not model full-body visuomotor coordination in natural settings. Bridging the gap between egocentric perception and full-body visuomotor learning remains an open challenge.  

We propose the first comprehensive predictive visuomotor learning framework, which jointly models head pose, gaze direction, and upper-body joint movements in 3D space. Unlike prior approaches that treat these signals independently\cite{jia2022generative,lai2022eye,liu2022joint}, our model explicitly captures their temporal dependencies by encoding kinematic sequences and generating future motion trajectories using a diffusion model. By conditioning on multimodal observations, our method learns structured visuomotor patterns, enabling more temporally consistent and accurate movement predictions.

Our approach is enabled by the recent emergence of the EgoExo4D \cite{grauman2024ego} and Nymeria \cite{ma2024nymeria} datasets, which contain comprehensive 3D annotations and make it possible to quantitatively evaluate visumotor forecasting performance. Specifically, we evaluate our approach on EgoExo4D, leveraging its 3D annotations of gaze, head pose, and body motion. Averaged over a 1-second forecasting horizon, our model achieves an average error of 59 mm for visuomotor translation (head position, gaze ray endpoint, and upper-body joints) and a head rotation error of 13 degrees, demonstrating promising performance across a diverse set of daily activities. By jointly modeling these visuomotor signals, our method provides deeper insights into their temporal dynamics, advancing the study of predictive human motion modeling.
Our contributions are summarized as follows: 
\begin{itemize}
    \item We define a unified visuomotor forecasting task that jointly predicts future head pose, gaze target and upper body motion from past egocentric visual and kinematic inputs.
    % \item We formulate a forecasting-based task for human visuomotor modeling, integrating head pose, gaze direction, fixation, and upper-body motion to capture temporal dependencies.
    \item We design a structured multimodal diffusion framework with separate head-gaze and head-gaze-arm pathways fused with visual context, providing conditioning that preserves cross modal visuomotor relations. 
    % \item We extend a diffusion-based framework that integrates egocentric vision and kinematic sequences, leveraging multimodal fusion to enhance temporal coherence and prediction accuracy.  
    \item We conduct thorough evaluations on the EgoExo4D dataset, demonstrating consistently strong performance across diverse real-world activities.  
    \item We provide detailed analyses and ablations that reveal concrete dependencies among head motion, gaze behavior and upper body dynamics in predictive coordination.
    % \item Our analysis includes extensive quantitative and qualitative evaluations, with a comprehensive ablation study assessing the impact of each multimodal component on accuracy.  
\end{itemize}


% \textbf{OLD INTRO}
% How visual context is transformed into motor acts by primate brains has been thoroughly studied in psychology and physiology~\cite{goodale1998visuomotor}. Moreover, studies underscore the predictive nature of visuomotor coordination, particularly in how visual memory informs motor planning. Hayhoe et al. \cite{hayhoe2003visual} observed that during natural tasks, individuals rely on visual information from previous fixations to plan and coordinate movements over seconds. A computational model for such anticipative visuomotor system can trigger new application or user experience in robotics and VR/AR, where anticipating human movement can enhance real-time decision-making and system adaptability.

% Humans operate in a visually rich world, where most actions depend on perceiving and interacting with the environment. At the core of this capability is the visuomotor system, which tightly couples head movements, gaze direction, and body coordination to facilitate task execution and adaptation. The complexity of this coordination varies across activities: some, like reaching for an object or navigating a space, require continuous visual-motor feedback, while others, such as typing or shooting a basketball, involve episodic synchronization, primarily during the planning phase. Additionally, high-precision tasks such as playing a musical instrument require suppressing natural visuomotor reflexes to maintain accuracy.

% Previous psychological research underscores the predictive nature of visuomotor coordination, particularly in how visual memory informs motor planning. Hayhoe et al. \cite{hayhoe2003visual} observed that during natural tasks like making a sandwich, individuals rely on visual information from previous fixations to plan and coordinate movements over several seconds. This reliance on stored visual memory allows humans to anticipate object locations and properties, ensuring seamless interaction with the environment. Understanding and modeling these predictive visuomotor behaviors is essential for robotics, VR/AR, and human-computer interaction, where anticipating human movement can enhance real-time decision-making and system adaptability.

% In robotics, visuomotor prediction has been explored to enhance manipulation and assistive tasks. Learning from human demonstrations \cite{finn2017one, lynch2019learning, zeng2020transporter} has enabled robots to generalize across diverse actions. However, these methods often rely on task-specific datasets and do not model full-body visuomotor coordination in natural settings.  

% Recent research has increasingly leveraged egocentric video analysis—first-person visual data captured by wearable cameras—to study visuomotor coordination. Deep learning models have been developed to forecast ego-motion, gaze, and hand trajectories from egocentric videos \cite{jia2022generative,lai2022eye,li2023ego}. However, most prior methods focus on isolated modality signals (e.g., only gaze or hand motion) and fail to model their multimodal interdependencies. A key limitation has been the lack of large-scale datasets with dense 3D annotations of full-body visuomotor dynamics. Recently, datasets such as EgoExo4D \cite{grauman2024ego} and Nymeria \cite{ma2024nymeria} have introduced comprehensive 3D annotations, enabling a holistic study of visuomotor coordination and its predictive nature in human movement.

% Despite these advancements, existing forecasting models remain limited in capturing multimodal dependencies in visuomotor coordination. To address this, we propose the first comprehensive visuomotor forecasting model, which jointly predicts head pose, gaze direction, and upper-body joint movements in 3D. Unlike prior approaches that treat these signals independently, our model explicitly captures their temporal dependencies by encoding kinematic sequences with a Transformer and generating future motion trajectories using a diffusion model. By conditioning on multimodal observations, our method produces more temporally consistent and accurate visuomotor forecasts.

% We evaluate our approach on EgoExo4D, leveraging its 3D annotations of gaze, head pose, and body motion. Averaged over a 1-second forecasting horizon, our model achieves an average error of 59 mm for visuomotor translation (head position, gaze ray endpoint, and upper-body joints) and a head rotation error of 13 degrees, demonstrating stable performance across diverse daily activities. By jointly modeling these visuomotor signals, our method provides deeper insights into their temporal dynamics, advancing the study of predictive human motion modeling.
% Our contributions are summarized as follows: 
% \begin{itemize}
%     \item We formulate a forecasting-based task for human visuomotor modeling, integrating head pose, gaze direction, fixation, and upper-body motion to capture temporal dependencies.
%     \item We extend a diffusion-based framework that integrates egocentric vision and kinematic sequences, leveraging multimodal fusion to enhance temporal coherence and prediction accuracy.  
%     \item We conduct extensive evaluations on the large-scale EgoExo4D dataset, demonstrating consistently strong performance across diverse real-world activities.  
%     \item Our analysis includes extensive quantitative and qualitative evaluations, with a comprehensive ablation study assessing the impact of each multimodal component on accuracy.  
% \end{itemize}


% \begin{itemize}
%     \item We propose a framework for human visuomotor modeling, capturing head pose, gaze direction, fixation, and upper-body motion. Given its predictive nature, we formulate this as a forecasting task to model temporal dynamics.  
%     % \item We extend a diffusion-based motion forecasting framework 
%     \item We extend a diffusion-based motion forecasting framework that integrates egocentric vision and kinematic sequences, capturing temporal dependencies for coherent and accurate motion prediction.  
%     % \item We introduce a multimodal diffusion-based forecasting model that integrates egocentric vision and kinematic sequences, capturing temporal dependencies for coherent and accurate motion prediction.  
%     \item We evaluate our model on the large-scale egocentric dataset EgoExo4D, demonstrating consistently strong performance across diverse daily activities.  
%     \item Our analysis includes extensive quantitative and qualitative evaluations with multiple metrics, alongside a rich ablation study to assess the contributions of each component.  
% \end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Humans operate in a visually rich world, where most actions depend on perceiving and interacting with the environment. At the core of this capability is the visuomotor system, which tightly couples head movements, gaze direction, and body coordination to facilitate task execution and adaptation. The complexity of this coordination varies across activities: some, like reaching for an object or navigating a space, require continuous visual-motor feedback, while others, such as typing or shooting a basketball, involve episodic synchronization, primarily during the planning phase. Additionally, high-precision tasks such as playing a musical instrument require suppressing natural visuomotor reflexes to maintain accuracy. Psychological research underscores the predictive nature of visuomotor coordination, highlighting how visual memory informs motor planning. For instance, Hayhoe et al.\cite{hayhoe2003visual} observed that during natural tasks like making a sandwich, individuals utilize visual information acquired from previous fixations to plan and coordinate movements over several seconds. This reliance on visual memory enables the anticipation of object locations and properties, facilitating seamless interaction with the environment. Understanding and modeling these predictive visuomotor behaviors is essential for fields such as robotics, VR/AR, and human-computer interaction, where anticipating human movement can enhance real-time decision-making and system adaptability.

% Recent research has increasingly leveraged egocentric video analysis—first-person visual data captured by wearable cameras—to study visuomotor coordination. Deep learning models have been developed to predict ego-motion, gaze, and hand trajectories from egocentric videos \cite{jia2022generative,lai2022eye,li2023ego}. However, most prior methods focus on isolated modality signals\cite{} (e.g., only gaze or hand motion) and fail to model their multimodal inter-dependencies. A major limitation has been the lack of large-scale datasets with dense 3D annotations of full-body visuomotor dynamics. Recently, datasets such as EgoExo4D \cite{grauman2024ego} and Nymeria \cite{ma2024nymeria} have introduced comprehensive 3D annotations, enabling a more holistic study of visuomotor coordination and its predictive nature in human movement.

% Despite these advancements, existing forecasting models remain limited in capturing the multimodal dependencies of visuomotor coordination. To address this, we propose the first comprehensive visuomotor forecasting model, which jointly predicts head pose, gaze direction, and upper-body joint movements in 3D. Unlike prior approaches that treat these signals independently, our model explicitly captures their temporal dependencies by encoding kinematic sequences with a Transformer and generating future motion trajectories using a diffusion model. By conditioning on multimodal observations, our method produces more temporally consistent and accurate visuomotor forecasts.

% We evaluate our approach on EgoExo4D, leveraging its 3D annotations of gaze, head pose, and body motion. Averaged over a 1-second forecasting horizon, our model achieves a PA-MPJPE of 59 mm for visuomotor translation (head position, gaze ray endpoint and upper-body joints) and a head rotation error of 14 degrees, demonstrating stable performance across diverse daily activities. By jointly modeling these visuomotor signals, our method produces temporally consistent and accurate predictions, providing deeper insights into their dynamics.

% Our contributions are summarized as follows: 
% \begin{itemize}
%     \item We propose a framework for human visuomotor modeling, capturing head pose, gaze direction, fixation, and upper-body motion. Given its predictive nature, we formulate this as a forecasting task to model temporal dynamics.  
%     \item We introduce a multimodal diffusion-based forecasting model that integrates egocentric vision and kinematic sequences, capturing temporal dependencies for coherent and accurate motion prediction.  
%     \item We evaluate our model on the large-scale egocentric dataset EgoExo4D, demonstrating consistently strong performance across diverse daily activities.  
%     \item Our analysis includes extensive quantitative and qualitative evaluations with multiple metrics, alongside a rich ablation study to assess the contributions of each component.  
% \end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We evaluate our approach on EgoExo4D, leveraging its comprehensive 3D annotations of gaze, head pose, and body motion to assess forecasting accuracy. Our model achieves a PA-MPJPE of X mm for upper-body motion and a gaze prediction error of Y degrees, demonstrating stable performance across diverse daily activities. Results show that jointly modeling these visuomotor signals leads to more accurate and temporally consistent predictions compared to treating them separately. By providing a structured approach to modeling visuomotor coordination, our work contributes to a deeper understanding of how gaze, head orientation, and upper-body motion evolve over time. 

% We evaluate our approach on EgoExo4D, leveraging its comprehensive 3D annotations of gaze, head pose, and body motion to assess forecasting accuracy. Our model achieves a PA-MPJPE of 59 mm for upper-body motion and a head rotation error of 14 degrees, demonstrating stable performance across diverse daily activities. By jointly modeling these visuomotor signals, our method produces more accurate and temporally consistent predictions. This structured approach to visuomotor coordination provides deeper insights into the temporal dynamics of gaze, head orientation, and upper-body motion.

% These insights lay the groundwork for future research in human-computer interaction and robot learning, where better predictions of human movement may enhance system responsiveness and coordination in interactive environments. 
% \begin{itemize}
%     % \item We introduce the first framework to jointly model and forecast a comprehensive 3D representation of human visuomotor coordination, encompassing head pose, gaze direction, gaze fixation, and upper-body motion.  
%     % \item We establish a comprehensive framework for human visuomotor modeling, capturing the coordination between head pose, gaze direction, and upper-body motion. Given the predictive nature of human visuomotor behavior, we formulate this as a forecasting task to model its temporal dynamics.  
%     \item We propose a framework for human visuomotor modeling, capturing head pose, gaze direction, gaze fixation, and upper-body motion. Given its predictive nature, we formulate this as a forecasting task to model temporal dynamics.
%     \item We introduce a multimodal diffusion-based forecasting model that integrates egocentric vision and kinematic sequences, capturing temporal dependencies for coherent and accurate motion prediction.  
%     \item We evaluate our model on the large-scale egocentric dataset EgoExo4D, demonstrating consistently strong performance across diverse daily activities.  
%     \item Our analysis includes extensive quantitative and qualitative evaluations with multiple metrics, along with a rich ablation study to assess the contributions of each component.  
%     % \item We present a multimodal diffusion-based forecasting model that integrates egocentric vision and kinematic sequences, capturing temporal dependencies for more coherent and accurate motion prediction.  
%     % \item We evaluate our model on the large-scale egocentric dataset EgoExo4D, demonstrating consistently strong performance across diverse daily activities.  
%     % \item Our analysis includes extensive quantitative and qualitative evaluations with multiple metrics, along with a rich ablation study to assess the contributions of each component.  
%     % \item We evaluate our model on the large-scale egocentric dataset EgoExo4D, demonstrating consistently strong performance across a diverse set of daily activities. Our analysis includes extensive. quantitative and qualitative evaluations with multiple metrics, along with a rich ablation study to provide further insight into the role of each component in our proposed visuomotor representation.
%     % \item We evaluate our model on the large-scale egocentric dataset EgoExo4D, demonstrating improved forecasting accuracy and temporal consistency compared to prior approaches across diverse skilled activities.
%     % \item We evaluate the proposed model on the large-scale egocentric datasets EgoExo4D. Quantitative and qualitative results demonstrate a strong generalization towards a wide range of daily skilled tasks.
% \end{itemize}

% Despite these advancements, existing forecasting models remain limited in capturing multimodal visuomotor dependencies. We introduce the first comprehensive visuomotor forecasting model, which jointly predicts head pose, gaze direction, gaze fixation, and upper-body joint movements in 3D. Unlike prior methods that model these signals in isolation, our approach learns their intrinsic relationships over time, improving the coherence and accuracy of future motion predictions. At its core, our framework employs a diffusion-based forecasting model, which effectively models the stochastic nature of human motion and generates consistent, multimodal future predictions. We evaluate our approach on EgoExo4D, leveraging its comprehensive 3D annotations of gaze, head pose, and body motion to assess forecasting accuracy. Results show that jointly modeling these visuomotor signals leads to more accurate and temporally consistent predictions compared to treating them separately. By providing a structured way to model the visuomotor system as an integrated whole, our work contributes to a deeper understanding of how gaze, head orientation, and upper-body motion evolve over time. These insights could inform future research in human-computer interaction and robot learning, where better predictions of human movement may improve system responsiveness and coordination in interactive environments.


% To evaluate our approach, we conduct large-scale experiments on EgoExo4D\cite{grauman2024ego}, assessing forecasting accuracy on head pose, gaze fixation, gaze direction, and body joint trajectories. Our results demonstrate that jointly modeling these visuomotor signals significantly outperforms approaches that treat them separately.

% Beyond advancing scientific understanding of human visuomotor coordination, our model has broad practical implications. In VR/AR, it enables more immersive and natural interactions by predicting user movements and adjusting virtual environments accordingly~\cite{lavoie2024comparing}. In robotics, our approach facilitates proactive human-robot collaboration in dynamic settings such as factories or hospitals, where robots can anticipate human movements to prevent collisions and optimize workflows.

% By modeling the full visuomotor system in 3D and leveraging probabilistic forecasting, our work lays a foundation for more sophisticated, human-aware AI systems, bringing us closer to naturalistic human-computer interactions and enhanced robotic autonomy.

% \begin{itemize}
%     \item We are the first to define a complete representation of the human visuomotor coordination system in 3D space. 
%     \item We present a multi-modal diffusion-based framework that forecasts the proposed visuomotor system.
%     % \item \color{red}
%     \item We evaluated the proposed model on the large-scale egocentric datasets EgoExo4D. Quantitative and qualitative results demonstrate a strong generalization towards a wide range of daily skilled tasks.
% \end{itemize}
% To insert a figure: \input{figs/template}
% Or table: \input{tables/template}
% \begin{figure*}[th]
%   \centering
%    \includegraphics[width=0.9\linewidth]{figs/teaser.png}
%    \caption{Given a sequence of egocentric frames with corresponding 3D poses, our target is to forecast the 3D poses in the next temporal window. }
%    \label{fig:visuomotor-system}
% \end{figure*}

==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related}

% \subsection{Human Visuomotor Coordination}
% \noindent \textbf{Human Visuomotor Coordination.}
% Human visuomotor coordination is fundamental to action planning and execution, integrating first-person perspective visual perception, head orientation, and proprioception to enable fluid, goal-directed movements. Unlike purely reactive control, it operates \textbf{\textit{predictively}}, allowing for smooth and adaptive actions despite sensory and neural delays \cite{nijhawan2009compensating,wolpert2001motor,shadmehr2010error, zago2009visuo,avraham2019effects}.
% Research in neuroscience and motor control highlights that head movement, gaze, and body posture work together to anticipate motion trajectories \cite{lappi2018visuomotor,land2001ways,bizzi1984posture}. Head orientation provides a stable spatial reference, aligning sensory input with motor execution, especially in dynamic environments\cite{graziano2006organization}. Proprioception further refines this process, allowing the brain to track limb positions and adjust movements accordingly\cite{shadmehr2008computational}. These multimodal cues are tightly coupled—humans naturally orient their head and upper body before executing reaching, stepping, or object manipulation tasks \cite{johansson2009coding}. This predictive integration is essential for both action preparation and real-time adaptation\cite{land2001ways,shadmehr2008computational}.

% Inspired by these biological mechanisms, our work explicitly integrates head orientation, gaze, and egocentric perception into motion forecasting, not as independent signals but bridging neuroscience insights with real-world human movement prediction as a structured visuomotor coordination representation. 


\noindent \textbf{Predictive Human Motion Modeling in Egocentric Vision.} 
Egocentric forecasting has been studied across several complementary modalities.
Gaze prediction approaches typically model 2D saliency or fixation likelihoods from past gaze trajectories and egocentric video~\cite{zhang2017deep,lai2022eye,lai2024listen}. Hand-trajectory forecasting focuses on predicting future hand motion in manipulation or interaction tasks~\cite{jia2022generative,liu2022joint,grauman2022ego4d}, while full-body forecasting from egocentric views models arm kinematics or activity-driven motion patterns~\cite{escobar2025egocast,chen2025egoagent}. Full-body forecasting has also been explored extensively in third-person settings~\cite{fragkiadaki2015recurrent,martinez2017human,pavllo2020modeling,mao2019learning,hernandez2019human,guo2023back}.
Although these works span rich prediction targets, they are generally single-modality formulations that do not model how gaze allocation, head motion, and upper-body dynamics interact over time.

A related direction uses gaze to inform motion prediction, such as walking or navigation behaviors constrained by scene geometry~\cite{kratzer2020mogaze,zheng2022gimo,yan2023gazemodiff,hu2024gazemotion}. However, these settings are dominated by environmental priors rather than internal visuomotor cues, and therefore capture a simpler form of gaze–motion coupling.

In contrast, upper-body actions such as reaching, manipulating, or fine-grained interaction require tight coordination between gaze, head orientation, and arm motion. Our work focuses on this setting, where multimodal dependencies arise from internal visuomotor control rather than external scene constraints.

\noindent \textbf{Visuomotor Coordination in Human Motor Control.}
Human visuomotor coordination integrates visual perception, head orientation, gaze allocation, and proprioceptive feedback into a predictive control loop~\cite{wolpert2001motor,shadmehr2008computational,nijhawan2009compensating,shadmehr2010error,zago2009visuo,avraham2019effects}. The motor system compensates for sensory and neural delays by building internal forward models and using recent visual information to anticipate the consequences of actions~\cite{shadmehr2010error,zago2009visuo,avraham2019effects}. Head orientation serves as a reference frame for stabilizing visual input and organizing posture for action~\cite{graziano2006organization,bizzi1984posture}. Gaze shifts reveal short-horizon task goals and are known to precede hand and arm movements during reaching, manipulation, and other visually guided behaviors~\cite{land2001ways,lappi2018visuomotor}. Proprioceptive signals refine arm trajectories and support rapid online corrections~\cite{johansson2009coding}. These findings consistently show that head, gaze, and upper-body dynamics evolve jointly rather than independently~\cite{land2001ways,shadmehr2008computational}, motivating our decision to model them as a coordinated visuomotor state.

% \noindent \textbf{Downstream Applications in HCI, AR, and Robotics.}
% \noindent \textbf{Downstream Applications.}
% Visuomotor Coordination in Interactive AI Systems
% Visuomotor Coordination in Embodied and Interactive AI
% Visuomotor Coordination in Human-Centered AI
% Visuomotor Coordination for Intention-Aware Systems

\noindent \textbf{Visuomotor Coordination in Embodied and Interactive AI.}
The coordination of head orientation, gaze behavior, and upper-body motion plays a central role across interactive AI settings including HCI, AR/VR, and robot manipulation. In HCI and AR/VR, head and gaze provide reliable cues about user intention and upcoming actions, supporting predictive interfaces and more responsive interaction~\cite{hayhoe2005eye,land2009looking,DavidJohn2021,Chen2022,Bisogni2024}. Systems that incorporate gaze-conditioned or viewpoint-aware representations have demonstrated improved contextual reasoning and enhanced responsiveness in smart-eyewear and AR applications~\cite{Konrad2024,Chen2022}. 
Robotics leverages similar principles: human gaze, foveated perception, and attention-driven representations improve manipulation performance and enable more robust visuomotor policies~\cite{finn2017one,zeng2020transporter,wang2021generalization,lynch2019learning,robomimic2021,zhu2023learning,kim2024openvla,black2024pi,aldaco2024aloha,jiang2024dexmimicgen}. However, natural head–gaze–body coupling is often suppressed in robot learning pipelines that rely on curated or “robot-like” demonstrations~\cite{bahl2022human,li2024okami,zhu2024vision,ren2025motion}, reducing the richness and generality of the resulting models~\cite{kerr2025eye,chuang2025look}. As a result, existing methods across these domains typically lack an explicit model of human visuomotor coordination.

Our work addresses this gap by predicting natural visuomotor coordination directly from in-the-wild human data~\cite{grauman2024ego}. By modeling the structured dependencies between head pose, 3D gaze endpoints, and upper-body motion, our framework provides data-driven insight into how visuomotor signals evolve together. This predictive representation can benefit future imitation learning, AR interaction, and gaze-conditioned AI systems by offering a principled way to incorporate natural coordination patterns into downstream models.
% \noindent \textbf{Downstream Applications in HCI, AR, and Robotics.}
% Understanding how head orientation, gaze behavior, and upper-body motion co-evolve is important for downstream applications in HCI, AR, and robotics. In HCI and AR/VR, head and gaze provide a powerful signal for user intention and predictive interaction\cite{hayhoe2005eye,land2009looking,DavidJohn2021,Chen2022,Bisogni2024}. Recent systems show that gaze-conditioned interfaces can significantly enhance contextual AI and smart eyewear performance\cite{Konrad2024}. Coordinated gaze and viewpoint have been shown to improve responsiveness and task performance in AR interaction\cite{Chen2022,DavidJohn2021}.

% Robotics research increasingly leverages similar principles. Vision-based manipulation systems benefit from integrating human gaze or foveated processing\cite{finn2017one,zeng2020transporter,wang2021generalization,lynch2019learning,robomimic2021,zhu2023learning,kim2024openvla,black2024pi,aldaco2024aloha,jiang2024dexmimicgen}. Kerr et al. show that an active foveated eye enables emergent eye–hand coordination and more robust manipulation\cite{kerr2025eye}, while Chuang et al. demonstrate that human-inspired gaze and foveated vision improve precision and robustness\cite{chuang2025look}. These works underscore the importance of modeling visuomotor structure for action planning.

% Natural human demonstrations, however, contain rich head–gaze–body coupling that current robot learning pipelines often suppress by encouraging “robot-like" demonstrations\cite{bahl2022human,li2024okami,zhu2024vision,ren2025motion}, which can limit generalization\cite{kerr2025eye,chuang2025look}. Our work provides a complementary direction by predicting natural visuomotor coordination directly from in-the-wild human data\cite{grauman2024ego}. Such predictive models offer data-driven insight into how humans allocate attention and coordinate actions, supporting future imitation learning, AR interaction, and gaze-conditioned AI systems.


% \noindent \textbf{Visuomotor Coordination in Human Motor Control.}
% Human visuomotor coordination integrates visual perception, head orientation, gaze allocation, and proprioceptive feedback into a predictive control loop\cite{wolpert2001motor,shadmehr2008computational,nijhawan2009compensating}.
% Head orientation serves as a reference frame for stabilizing visual input and aligning perception with planned motor actions\cite{graziano2006organization}.
% Gaze shifts reveal short-horizon task goals and are known to precede hand motion during reaching, manipulation, or visually guided tasks\cite{land2001ways,lappi2018visuomotor}.
% Proprioceptive signals refine arm trajectories and support rapid online correction\cite{johansson2009coding}.
% These findings consistently show that head, gaze, and upper-body dynamics evolve jointly rather than independently.

% This body of evidence motivates modeling visuomotor behavior as a coordinated multimodal process.
% Instead of predicting gaze, head motion, or arms separately, a unified representation enables the learning of spatial and temporal dependencies across perceptual and motor pathways.
% Our formulation draws directly from this literature by integrating head pose, gaze direction, and upper-body joints into a single visuomotor state whose future evolution reflects these coordinated mechanisms.

% \noindent \textbf{Bridging Visuomotor and Imitation Learning.}
% Robotic imitation learning seeks to acquire skills from human demonstrations\cite{finn2017one,lynch2019learning,zeng2020transporter,robomimic2021}.
% Recent methods explore learning from human videos\cite{kareer2024egomimic,kim2024openvla}, but many datasets instruct demonstrators to reduce natural head and body movement for policy simplicity\cite{bahl2022human,li2024okami,zhu2024vision}.
% This simplification removes the rich couplings between gaze, head pose, and arm motion that characterize natural visuomotor behavior.
% Consequently, imitation learning frameworks often lack signals that explain where attention is allocated or how actions are planned relative to head–gaze cues.

% Our work contributes to this direction by providing a predictive model of human visuomotor coordination, capturing the structured dependencies between head pose, gaze, and upper-body motion. Unlike imitation learning approaches that focus on end-to-end policy learning, our model predicts natural visuomotor behavior from in-the-wild datasets \cite{grauman2024ego}. By explicitly modeling visuomotor coordination, our framework can serve as a foundation for future imitation learning research, providing data-driven insights into human movement dynamics that can improve robot learning from human demonstrations.

% % \subsection{Bridging Visuomotor and Imitation Learning}
% \noindent \textbf{Bridging Visuomotor and Imitation Learning.}
% Recent advances in visuomotor imitation learning have enabled robots to acquire complex skills from human demonstrations \cite{finn2017one,zeng2020transporter,wang2021generalization,lynch2019learning,robomimic2021,zhu2023learning,kim2024openvla,black2024pi,aldaco2024aloha,jiang2024dexmimicgen}. Works like EgoMimic \cite{kareer2024egomimic} explore direct learning from human video data, removing the need for explicit robot data collection. However, modeling human visuomotor coordination remains a challenge, as it involves intricate couplings between gaze, head, and body movements that reflect hidden decision-making processes \cite{lin2025sim}.  

% To simplify learning, many existing methods instruct demonstrators to behave ``robot-like" by minimizing natural head and body movements \cite{bahl2022human,li2024okami,zhu2024vision,ren2025motion}. While effective for policy learning, this approach loses the richness of natural human behavior, making it difficult to generalize beyond constrained demonstrations. \cite{kerr2025eye,chuang2025look}

% Our work contributes to this direction by providing a predictive model of human visuomotor coordination, capturing the structured dependencies between head pose, gaze, and upper-body motion. Unlike imitation learning approaches that focus on end-to-end policy learning, our model predicts natural visuomotor behavior from in-the-wild datasets \cite{grauman2024ego}. By explicitly modeling visuomotor coordination, our framework can serve as a foundation for future imitation learning research, providing data-driven insights into human movement dynamics that can improve robot learning from human demonstrations.



==> sec/2_related_old.tex <==
\section{Related Work}
\label{sec:related}

% \subsection{Egocentric Vision and Visuomotor Prediction}
% \subsection{Visuomotor Prediction in Egocentric Vision}
% {\color{blue}{\subsection{Human Visuomotor Coordination}}}
\subsection{Human Visuomotor Coordination}

Human visuomotor coordination is fundamental to action planning and execution, integrating first-person perspective visual perception, head orientation, and proprioception to enable fluid, goal-directed movements. Unlike purely reactive control, it operates \textbf{\textit{predictively}}, allowing for smooth and adaptive actions despite sensory and neural delays \cite{nijhawan2009compensating,wolpert2001motor,shadmehr2010error, zago2009visuo,avraham2019effects}.
Research in neuroscience and motor control highlights that head movement, gaze, and body posture work together to anticipate motion trajectories \cite{lappi2018visuomotor,land2001ways,bizzi1984posture}. Head orientation provides a stable spatial reference, aligning sensory input with motor execution, especially in dynamic environments\cite{graziano2006organization}. Proprioception further refines this process, allowing the brain to track limb positions and adjust movements accordingly\cite{shadmehr2008computational}. These multimodal cues are tightly coupled—humans naturally orient their head and upper body before executing reaching, stepping, or object manipulation tasks \cite{johansson2009coding}. This predictive integration is essential for both action preparation and real-time adaptation\cite{land2001ways,shadmehr2008computational}.

Inspired by these biological mechanisms, our work explicitly integrates head orientation, gaze, and egocentric perception into motion forecasting, not as independent signals but bridging neuroscience insights with real-world human movement prediction as a structured visuomotor coordination representation. 

\subsection{Modeling Predictive Visuomotor Coordination}

Existing human motion forecasting methods often focus on isolated sub-components rather than their integration. Gaze forecasting predicts future fixation points from past gaze trajectories, often using egocentric video \cite{zhang2017deep,lai2022eye,lai2023listen}, but it does not model how gaze directs motor actions. Hand trajectory forecasting predicts hand motion in first-person views, typically for object interactions \cite{liu2022joint,jia2022generative,grauman2022ego4d}, yet it largely ignores head movement and body posture, which naturally influence hand coordination. Full-body motion forecasting predicts skeletal motion based on past joint positions \cite{fragkiadaki2015recurrent,martinez2017human,pavllo2020modeling,mao2019learning,hernandez2019human,guo2023back,chen2023humanmac}, but lower-body motion is often dictated by external terrain constraints rather than internal visuomotor coordination. In contrast, upper-body motion is directly linked to fine motor tasks, object interactions, and skill-based activities, where visuomotor coordination plays a critical role. Thus, we focus on \textbf{\textit{upper-body dynamics}}, ensuring our approach remains independent of environmental priors while maintaining relevance across diverse skilled activities.  

Egocentric vision has emerged as a key modality for studying human visuomotor coordination, as it provides a first-person perspective of perception and action. Unlike third-person views, egocentric video directly captures the relationship between visual attention, head movement, and motor execution, making it well-suited for modeling predictive visuomotor behaviors \cite{zhang2017deep,jia2022generative,li2023ego,tan2023egodistill}. This perspective is particularly valuable for understanding how humans coordinate gaze, head, and body movements in dynamic environments.  

Another line of research incorporates environmental cues for motion prediction. Gaze-informed full-body forecasting has been explored in navigation tasks, using gaze to anticipate walking trajectories \cite{kratzer2020mogaze,zheng2022gimo,yan2023gazemodiff,hu2024gazemotion}. However, these tasks are simpler, as locomotion follows scene constraints rather than requiring complex visuomotor coordination. Full-body forecasting in interactive activities integrates environmental affordances to predict human motion \cite{zheng2022gimo,ashutosh2024fiction}, but such methods heavily rely on external cues like object locations or scene semantics, making them less generalizable to unstructured or unseen environments.  

In contrast, our work addresses a more complex and generalizable problem by unifying head orientation, gaze, and upper-body motion as predictive signals for motion forecasting. By focusing primarily on internal visuomotor cues, our model learns a biologically grounded representation applicable across diverse activities, without explicitly relying on structured environmental priors.


% \subsection{Visuomotor Coordination in Imitation Learning}
\subsection{Bridging Visuomotor and Imitation Learning}
Recent advances in visuomotor imitation learning have enabled robots to acquire complex skills from human demonstrations \cite{finn2017one,zeng2020transporter,wang2021generalization,lynch2019learning,robomimic2021,zhu2023learning,kim2024openvla,black2024pi,aldaco2024aloha,jiang2024dexmimicgen}. Works like EgoMimic \cite{kareer2024egomimic} explore direct learning from human video data, removing the need for explicit robot data collection. However, modeling human visuomotor coordination remains a challenge, as it involves intricate couplings between gaze, head, and body movements that reflect hidden decision-making processes \cite{lin2025sim}.  

To simplify learning, many existing methods instruct demonstrators to behave ``robot-like" by minimizing natural head and body movements \cite{bahl2022human,li2024okami,zhu2024vision,ren2025motion}. While effective for policy learning, this approach loses the richness of natural human behavior, making it difficult to generalize beyond constrained demonstrations.  

Our work contributes to this direction by providing a predictive model of human visuomotor coordination, capturing the structured dependencies between head pose, gaze, and upper-body motion. Unlike imitation learning approaches that focus on end-to-end policy learning, our model predicts natural visuomotor behavior from in-the-wild datasets \cite{grauman2024ego}. By explicitly modeling visuomotor coordination, our framework can serve as a foundation for future imitation learning research, providing data-driven insights into human movement dynamics that can improve robot learning from human demonstrations.




% traditional motion forecasting approaches that predict skeletal trajectories in isolation\cite{chiu2019action,chen2023humanmac,guo2023back,}, visuomotor coordination inherently involves structured dependencies between head pose, gaze, and upper-body movement, making it crucial for understanding human intent and interaction.


% Human visuomotor coordination is fundamental to action planning and execution, as it inherently involves structured dependencies between head pose, gaze, and upper-body movement, 

% integrating visual perception, head orientation, and proprioception to enable fluid, goal-directed movements. Unlike purely reactive control, it operates \textbf{\textit{predictively}}, allowing for smooth and adaptive actions despite sensory and neural delays \cite{nijhawan2009compensating,wolpert2001motor,shadmehr2010error, zago2009visuo,avraham2019effects}.

% This differs from traditional forecasting tasks, where full-body skeletal prediction is the primary goal. Instead, our focus is on modeling how visuomotor elements coordinate in upper-body tasks, where head-gaze-hand synchronization plays a critical role.

% Despite these insights, computational models for human motion prediction often treat pose forecasting as an isolated sequence modeling task, neglecting the rich multimodal interactions that shape human movement. Some recent methods have leveraged gaze for motion forecasting \cite{}, but these approaches primarily rely on simulated data or focus on navigation-based behaviors, rather than complex, skilled activities such as object manipulation, sports, or assembly tasks. A more comprehensive framework is needed to capture the predictive role of head orientation, gaze, and egocentric perception in fine-grained human actions.

% Our work addresses this gap by explicitly modeling visuomotor coordination as a predictive process, integrating head movement, gaze, and egocentric cues into a motion forecasting framework. This biologically inspired approach aligns with human motor behavior, enabling more accurate and temporally coherent predictions of future movement.

% Human visuomotor coordination plays a fundamental role in action planning and execution, integrating visual perception with motor control to facilitate smooth and adaptive movements. Prior research has extensively explored this coordination in various domains, including neuroscience, cognitive science, and computer vision.

% \subsection{Visuomotor Prediction in Egocentric Vision}
% \subsection{Vision-Based Human Motion Forecasting}
% {\color{blue}{\subsection{Visuomotor Motion Forecasting}}}
% Egocentric vision has emerged as a key modality for studying human visuomotor coordination, as it provides a first-person perspective of perception and action. Unlike third-person views, egocentric video directly captures the relationship between visual attention, head movement, and motor execution, making it well-suited for modeling predictive visuomotor behaviors\cite{zhang2017deep,jia2022generative,li2023ego,tan2023egodistill}. This perspective is particularly valuable for understanding how humans plan and execute actions in dynamic environments, where gaze and head pose play a crucial role in guiding motor behavior.

% Existing approaches to human motion forecasting typically focus on isolated sub-components of visuomotor coordination, modeling gaze, hand trajectories, or full-body motion separately rather than as an integrated system, which is fundamental to human motion planning. Gaze forecasting predicts future fixation points from past gaze trajectories, often using egocentric video \cite{zhang2017deep,lai2022eye,lai2023listen}. While useful for understanding attention, these models do not capture how gaze actively influences motor actions. Hand trajectory forecasting predicts hand motion in first-person views, typically for object interactions \cite{liu2022joint,jia2022generative,grauman2022ego4d}. However, these methods rarely account for head movement and body posture, which naturally influence hand coordination. Full-body motion forecasting focuses on predicting skeletal motion based on past joint positions \cite{fragkiadaki2015recurrent,martinez2017human,pavllo2020modeling,mao2019learning,hernandez2019human,guo2023back,chen2023humanmac}. While effective for general motion dynamics, lower-body movement is often dictated by external terrain constraints and locomotion objectives, making it less dependent on internal visuomotor coordination. In contrast, upper-body motion is directly linked to fine motor tasks, object interactions, and skill-based activities, where visuomotor coordination plays a critical role. Thus, we focus exclusively on \textbf{\textit{upper-body dynamics}}, ensuring that our approach remains independent of environmental priors while maintaining relevance across diverse skilled activities.

% Another line of research incorporates \textit{environmental cues} for motion prediction. Gaze-informed full-body forecasting has been explored in navigation tasks, leveraging gaze information to anticipate walking trajectories \cite{kratzer2020mogaze,zheng2022gimo,yan2023gazemodiff,hu2024gazemotion}. However, these tasks are relatively simpler, as locomotion primarily follows scene constraints rather than requiring complex visuomotor coordination. Similarly, full-body forecasting in interactive activities incorporates environmental affordances to predict human motion \cite{zheng2022gimo,ashutosh2024fiction}, but these approaches rely heavily on external context such as object locations or scene semantics, making them less generalizable in unstructured or unseen environments.  In contrast, our work tackles a more complex and generalizable problem by unifying head orientation, gaze, and upper-body motion as predictive signals for motion forecasting. By focusing solely on internal visuomotor cues rather than external environmental priors, our model learns a biologically grounded representation that is applicable across diverse activities, without assuming the presence of structured external information.  

% Egocentric vision has emerged as a key modality for studying human visuomotor coordination, as it provides a first-person perspective of perception and action. Unlike third-person views, egocentric video directly captures the relationship between visual attention, head movement, and motor execution, making it well-suited for modeling predictive visuomotor behaviors \cite{zhang2017deep,jia2022generative,li2023ego,tan2023egodistill}. This perspective is particularly valuable for understanding how humans coordinate gaze, head, and body movements in dynamic environments.  

% Existing human motion forecasting methods often focus on isolated sub-components rather than their integration. Gaze forecasting predicts future fixation points from past gaze trajectories, often using egocentric video \cite{zhang2017deep,lai2022eye,lai2023listen}, but it does not model how gaze directs motor actions. Hand trajectory forecasting predicts hand motion in first-person views, typically for object interactions \cite{liu2022joint,jia2022generative,grauman2022ego4d}, yet it largely ignores head movement and body posture, which naturally influence hand coordination. Full-body motion forecasting predicts skeletal motion based on past joint positions \cite{fragkiadaki2015recurrent,martinez2017human,pavllo2020modeling,mao2019learning,hernandez2019human,guo2023back,chen2023humanmac}, but lower-body motion is often dictated by external terrain constraints rather than internal visuomotor coordination. In contrast, upper-body motion is directly linked to fine motor tasks, object interactions, and skill-based activities, where visuomotor coordination plays a critical role. Thus, we focus on \textit{\textbf{upper-body dynamics}}, ensuring our approach remains independent of environmental priors while maintaining relevance across diverse skilled activities.  

% Another line of research incorporates environmental cues for motion prediction. Gaze-informed full-body forecasting has been explored in navigation tasks, using gaze to anticipate walking trajectories \cite{kratzer2020mogaze,zheng2022gimo,yan2023gazemodiff,hu2024gazemotion}. However, these tasks are simpler, as locomotion follows scene constraints rather than requiring complex visuomotor coordination. Full-body forecasting in interactive activities integrates environmental affordances to predict human motion \cite{zheng2022gimo,ashutosh2024fiction}, but such methods heavily rely on external cues like object locations or scene semantics, making them less generalizable to unstructured or unseen environments.  

% In contrast, our work addresses a more complex and generalizable problem by unifying head orientation, gaze, and upper-body motion as predictive signals for motion forecasting. By focusing primarily on internal visuomotor cues, our model learns a biologically grounded representation applicable across diverse activities, without explicitly relying on structured environmental priors.

% In contrast, our work addresses a more complex and generalizable problem by unifying head orientation, gaze, and upper-body motion as predictive signals for motion forecasting. By focusing solely on internal visuomotor cues, our model learns a biologically grounded representation applicable across diverse activities, without assuming structured environmental information.  

% In contrast, our work addresses a more complex and generalizable problem by unifying head orientation, gaze, and upper-body motion as predictive signals for motion forecasting. By integrating egocentric vision with internal visuomotor cues, our model learns a biologically grounded representation applicable across diverse activities, without explicitly encoding structured environmental priors.

% \subsection{From Isolated Signals to Visuomotor Integration}

% separate modeling: 2D gaze forecasting, 2D hand forecasting, 3D full body forecasting. In contrast: our work joint model the entire visuomor system. 

% joint modeling with environment cue: 3D gaze-informed full body forecasting (navigation, full body), 3D full body forecasting (interactive activity).  In contrast: our work focus only on the human visuomotor signal itself, regardless extra environment cue. 
% Another line of research incorporates environmental cues for motion prediction. Gaze-informed full-body forecasting has been explored in navigation tasks, leveraging gaze information to anticipate walking trajectories \cite{kratzer2020mogaze,zheng2022gimo,yan2023gazemodiff,hu2024gazemotion}. Similarly, full-body forecasting in interactive activities incorporates environmental affordances to predict human motion in interactive tasks \cite{zheng2022gimo,ashutosh2024fiction}. While these methods improve motion reasoning in structured environments, they rely heavily on external context, making them less generalizable where such information is unavailable. In contrast, our work unifies visuomotor coordination by jointly modeling \textbf{\textit{head orientation, gaze, and upper-body motion}} as predictive signals for motion forecasting. By focusing solely on internal visuomotor cues rather than external environmental priors, our model offers a generalizable, biologically inspired approach to human motion prediction.

% {\color{red}{\subsection{Visuomotor Policy Learning}}}
% \subsection{Visuomotor Imitation Learning}
% In this work, we study the core problem of learning human behavior prediction models from in-the-wild datasets~\cite{grauman2024ego}, focusing specifically on forecasting visuomotor coordination states. Unlike prior approaches that treat gaze, head movement, and body motion as independent phenomena~\cite{}, our framework explicitly models their coordinations. By aligning the input sensory signals (image, proprioception) and output space (motion trajectories) with that of a visuomotor policy, we hope to inform future researchers of the challenges and opportunities in learning behavior models from egocentric human data.


% \subsection{Visuomotor Learning in Embodied AI}
% visuomotor is a valuable topic in vision-based robot learning for task planning and execution. 
% egocentric vision has emerged as a powerful tool for robot learning human skills from a human's perspective. 
% diffusion model serves as a powerful tool to process multimodal data conditioned from both the vision source and kinematic data. 
% our work use diffusion based model to learn from multimodal human visuomotor data, and potentially benefit human-robot skill/coordination transfer (?) and collabration. 

% Training visuomotor policies from teleoperated demonstrations have shown remarkable potential in enabling robots to perform complex tasks. More recent works have investigated into directly learning from human video data to further scale up learning. For example, EgoMimic~\cite{} has shown. 
% However, unlike imitating teleoperated demonstrations, directly learning predictive models from egocentric human data remains a challenging problem due to the complex visuomotor coordination behaviors that reflect the hidden decision making ... of the humans. As a result, existing works often instruct the demonstrator to behave ``robot-like'' by minimizing head and full-body motion. In this work, we study the core problem of learning human behavior prediction models from in-the-wild dataset.  By aligning the input sensory signal (image, proprioception) and output space (trajectory prediction) of the learning problem setup, we hope to shed new light on how ... 

% Visuomotor learning is fundamental in embodied AI, enabling agents to perceive and generate coordinated motor actions~\cite{}. Understanding how vision and motion interact is crucial for skill acquisition, action prediction, and task execution, particularly in applications such as assistive robotics and human-robot collaboration~\cite{}.

% Egocentric vision has recently emerged as a powerful modality for visuomotor learning, offering a first-person perspective that naturally captures attentional focus and motion intent~\cite{grauman2022ego4d, li2022egoexo}. Unlike third-person observations, egocentric data provides direct insight into where a subject is looking, how they interact with objects, and how their movements unfold~\cite{kazuhiro2019gaze, land1999gaze}. This makes it particularly suitable for modeling visuomotor coordination in real-world tasks, from object manipulation to full-body motion prediction~\cite{kareer2024egomimic}.

% Our work builds on these advancements by learning visuomotor coordination from human demonstrations, integrating egocentric visual cues with kinematic observations. By capturing the intricate relationships between gaze, head pose, and upper-body motion, our model enhances motion prediction accuracy and has the potential to facilitate human-robot skill transfer and collaboration.


% Visuomotor learning is a fundamental topic in vision-based robot learning, enabling intelligent agents to plan and execute tasks by understanding the relationship between perception and action~\cite{}. A key challenge in this domain is effectively modeling the coordination between visual inputs and motor control to facilitate skill learning, imitation, and real-world interaction.

% Egocentric vision has emerged as a powerful tool for learning human skills from a first-person perspective~\cite{grauman2022ego4d, li2022egoexo}. By capturing observations from the viewpoint of an acting agent, egocentric data provides rich information about attentional focus, motion intent, and interaction dynamics~\cite{kareer2024egomimic}. This perspective is particularly beneficial for modeling human visuomotor coordination, as it inherently encodes spatial awareness and gaze-driven action planning~\cite{}.

% Recent advances in diffusion models have demonstrated strong capabilities in processing multimodal data by learning complex distributions over temporal sequences~\cite{ho2020denoising, yang2023diffusion}. In the context of visuomotor learning, diffusion-based approaches provide a flexible framework for forecasting future states conditioned on both egocentric vision and kinematic inputs~\cite{chi2023diffusion}. This allows for improved motion prediction, uncertainty modeling, and the generation of coherent action sequences.

% Our work builds on these advancements by employing a diffusion-based model to learn from multimodal human visuomotor data, integrating egocentric visual cues with kinematic observations. By capturing the intricate relationships between gaze, upper-body motion, and future action trajectories, our approach has the potential to benefit human-robot skill transfer, coordination learning, and collaborative task execution.


% In contrast, our work unifies visuomotor coordination by jointly modeling \textbf{head orientation, gaze, and upper-body motion} as predictive signals for motion forecasting. By focusing solely on internal visuomotor cues rather than external environmental priors, our model offers a generalizable, biologically inspired approach to human motion prediction.

% Existing approaches to human motion forecasting typically focus on isolated visuomotor signals\cite{} or incorporate external environmental cues to improve prediction\cite{}. However, these methods fail to model the internal coordination between gaze, head orientation, and body movement, which is fundamental to human motion planning.

% Many existing works focus on separately predict 2D gaze, 2D hand trajectories, or 3D full-body motion. Gaze forecasting predicts future fixation points based on past eye movements, often using egocentric video \cite{}. While useful for understanding attention, these models do not capture how gaze influences motor actions. Hand trajectory forecasting focuses on predicting hand motion in first-person views, typically for object interactions \cite{}. These approaches often ignore the role of head movement and body posture, which naturally influence hand coordination. Meanwhile, 3D full-body forecasting predicts skeletal motion based on past joint positions \cite{}, but does not integrate gaze and head orientation, missing key predictive cues present in human visuomotor coordination.



% Human motion forecasting has traditionally focused on predicting body pose sequences from past joint positions, often treating it as an isolated sequence modeling task. Some recent methods incorporate gaze as a predictive cue, but these approaches primarily rely on simulated data\cite{hu2024gazemotion} or focus on navigation-based behaviors\cite{zheng2022gimo}, neglecting complex, skilled activities such as object manipulation, sports, or assembly tasks. A more comprehensive framework is needed to model how head orientation, gaze, and egocentric perception jointly contribute to human motion prediction. 

% Egocentric vision has emerged as a powerful paradigm for understanding and predicting human actions from a first-person perspective. Prior work in ego-motion prediction focuses on forecasting body movements from egocentric video streams. Early methods relied on optical flow and hand-crafted motion features \cite{kitani2011activity}, while more recent deep learning approaches use transformers and recurrent architectures to model visuomotor dependencies \cite{}. However, these approaches primarily exploit visual motion cues rather than explicitly integrating predictive visuomotor signals.  


% Egocentric vision has emerged as a powerful paradigm in computer vision, enabling models to analyze and predict human actions based on first-person observations. Prior works have explored ego-motion prediction, focusing on forecasting future body movements from egocentric video streams. Traditional approaches rely on optical flow and hand-crafted motion features\cite{kitani2011activity}, while recent deep learning-based methods leverage transformers and recurrent architectures to model long-term dependencies\cite{li2023ego, jia2022generative}.
% A key challenge in ego-motion prediction is the multimodal nature of visuomotor coordination. Some works focus on gaze-based forecasting, predicting future gaze fixations from past gaze trajectories~\cite{huang2018predicting, assens2018pathgan}, while others focus on hand or limb movement prediction using wearable sensors or vision-based tracking~\cite{fathi2012learning, li2021gaze}. However, these methods typically model only a single modality, such as gaze or hand motion, without capturing their joint dependencies within the visuomotor system.
% Previous work primarily focuses on full-body motion or action recognition, with limited emphasis on the coordination between gaze, head, and upper-body movement, which is central to visuomotor tasks.

% \subsection{Visuomotor Prediction for Embodied AI and Robotics}


% \subsection{Multimodal Human Motion Forecasting}

% Human motion forecasting aims to predict future body poses and actions from historical observations. Traditional kinematic models employ Markovian and physics-based formulations\cite{taylor2007modeling}, while modern approaches adopt deep recurrent networks\cite{martinez2017human} and diffusion-based models~\cite{tevet2023human} for more flexible, data-driven predictions.

% Recent advancements in multimodal motion forecasting integrate information from pose, gaze, and scene context to improve prediction quality~\cite{yuan2023neural, grauman2024ego}. Notably, Nymeria\cite{ma2024nymeria} and EgoExo4D\cite{grauman2024ego} introduce large-scale datasets that densely capture head, gaze, and body motion, enabling comprehensive visuomotor learning. However, existing models often lack the ability to jointly model these modalities in a unified framework.


% \subsection{Future Action Guidance in Motion Prediction}

% Predicting human motion based solely on past observations can be ambiguous, as multiple plausible futures exist. To address this, researchers have explored intent-driven forecasting, where models incorporate task-related cues to improve prediction accuracy~\cite{goyal2019inferring}. Some approaches leverage text-based future action descriptions to guide motion generation~\cite{ahn2022can, shen2023action}, enabling models to anticipate actions based on human intent rather than just low-level dynamics.

% Despite these advancements, prior works either focus on single-modality forecasting or lack explicit future action conditioning. Our work bridges this gap by proposing a diffusion-based visuomotor forecasting model that jointly predicts head pose, gaze, gaze fixation, and body joints, while being guided by future action descriptions. This enables task-aware and multimodal motion forecasting, significantly improving prediction accuracy in egocentric scenarios.





==> sec/3_method.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=0.9\linewidth]{figs/vcr.png}
   \caption{Visualizing the Visuomotor Coordination Representation by mapping it onto a human mesh for better interpretability.}
   \label{fig:visuomotor-rep}
    \vspace{-12pt}
\end{figure}

\section{Method}
\label{sec:method}
We first introduce the \textit{Visuomotor Coordination Representation} and its corresponding visuomotor state (Sec.~\ref{subsec:vcr}), then formalize the forecasting objective (Sec.~\ref{subsec:forecasttask}). We next describe the canonicalization step that enforces spatial and temporal consistency (Sec.~\ref{subsec:canonicalization}), and finally present the diffusion-based prediction framework (Sec.~\ref{subsec:arch}).
% We define the \textit{Visuomotor Coordination Representation} (Sec.~\ref{subsec:vcr}) and introduce the forecasting task (Sec.~\ref{subsec:forecasttask}). To remove absolute head motion and ensure temporal and spatial consistency, we apply a state canonicalization process (Sec.~\ref{subsec:canonicalization}). We present our diffusion-based generative framework for visuomotor learning in (Sec.~\ref{subsec:arch}).  

% We define the \textit{Visuomotor Coordination Representation} (Sec.~\ref{subsec:vcr}) and introduce the forecasting task (Sec.~\ref{subsec:forecasttask}). To mitigate motion noise caused by camera movement, we apply a state canonicalization process (Sec.~\ref{subsec:canonicalization}). We present our diffusion-based generative framework for visualmotor learning in (Sec.~\ref{subsec:arch}).  

\subsection{Human Visuomotor Representation}
\label{subsec:vcr}

Human visuomotor coordination involves three key components: the \textbf{\textit{head pose}}, which establishes a spatial reference frame; the \textbf{\textit{gaze point}}, which reflects visual attention and intent; and the \textbf{\textit{upper-body joints}}, which provide motion cues relevant to interaction and task execution. We refer to this set of components collectively as the \textit{Visuomotor Coordination Representation (VCR)}.
At each timestep, the VCR defines a \textit{visuomotor state}
% At each time step, we instantiate the VCR as a \textit{visuomotor state}
\[
S_t = \{H_t, G_t, U_t\},
\]
where $H_t = (\mathbf{p}_{head}, \mathbf{R}_{head})$ denotes the head position $\mathbf{p}_{head} \in \mathbb{R}^3$ and orientation $\mathbf{R}_{head} \in SO(3)$. The gaze component $G_t$ is represented by the gaze endpoint $\mathbf{g} = \mathbf{p}_{head} + \lambda \mathbf{d}_{gaze}$, where $\mathbf{d}_{gaze}$ is the unit gaze direction derived from $\mathbf{R}_{head}$ and $\lambda$ is a fixed ray length. The upper-body joints $U_t = \{\mathbf{j}_i \in \mathbb{R}^3 \mid i = 1,\dots,6\}$ include the positions of shoulders, elbows, and wrists. Figure \ref{fig:visuomotor-rep} visualizes the Visuomotor Coordination Representation on a human mesh together with the corresponding egocentric frame.

% To effectively capture human visuomotor coordination, we consider three essential components: the \textit{head pose}, which establishes a spatial reference frame for movement; the \textit{gaze point}, which serves as an indicator of visual attention and intent; and the \textit{upper-body joints}, which provide motion cues relevant to interaction and task execution. These components collectively define the \textit{Visuomotor Coordination Representation (VCR)} by encapsulating the key factors that drive human visuomotor behavior.

% We formally define: \(VCR = \{ H, G, U \}\), where \( H = (\mathbf{p}_{head}, \mathbf{R}_{head}) \) represents the head pose with position \( \mathbf{p}_{head} \in \mathbb{R}^3 \) and orientation \( \mathbf{R}_{head} \in SO(3) \), \( G = \mathbf{g} \) denotes the endpoint of a fixed-length vector originating from the head position representing gaze ray,  with \( \mathbf{g} \in \mathbb{R}^3 \), and \( U = \{ \mathbf{j}_i \in \mathbb{R}^3 \mid i = 1, \dots, 6 \} \) represents the upper-body joint positions, including shoulders, elbows, and wrists. \cref{fig:visuomotor-rep} visualizes an example of VCR from Nymeria~\cite{ma2024nymeria}.

% \cref{fig:visuomotor-rep} shows an example visuomotor state from Nymeria~\cite{ma2024nymeria}.

% We formally define a visuomotor state: \( S = \{ H, G, U \} \), where \( H = (\mathbf{p}_{head}, \mathbf{R}_{head}) \) represents the head pose with position \( \mathbf{p}_{head} \in \mathbb{R}^3 \) and orientation \( \mathbf{R}_{head} \in SO(3) \). The gaze component \( G \) is represented by the \textit{gaze endpoint} \( \mathbf{g} \), defined as \(\mathbf{g} = \mathbf{p}_{head} + \lambda \mathbf{d}_{gaze}\), where \( \mathbf{d}_{gaze} \in \mathbb{R}^3 \) is the unit gaze direction derived from \( \mathbf{R}_{head} \), and \( \lambda \) is a predefined scalar controlling the gaze ray length. Finally, \( U = \{ \mathbf{j}_i \in \mathbb{R}^3 \mid i = 1, \dots, 6 \} \) represents the upper-body joint positions, including shoulders, elbows, and wrists. \cref{fig:visuomotor-rep} visualizes an example of VCR from Nymeria~\cite{ma2024nymeria}.

\subsection{Visuomotor State Forecasting}
\label{subsec:forecasttask}

Given a sequence of visuomotor states
\(
S_{t-\tau:t} = \{S_{t-\tau}, \dots, S_t\},
\)
together with its corresponding egocentric video clip
$E \in \mathbb{R}^{C \times T \times H \times W}$, the goal is to predict the
future visuomotor states $\hat{S}_{t+1:t+\Delta}$ over a horizon of $\Delta$
steps. This requires modeling the temporal evolution of head pose, gaze, and
upper-body joint dynamics conditioned on past kinematic and visual cues.

Formally, we define the \textit{Visuomotor Forecasting Task} as learning a
function
\vspace{-6pt}
\[
\hat{S}_{t+1:t+\Delta}
    = f(S_{t-\tau:t},\, E_{t-\tau:t}),
 \]
% \vspace{-3pt}
where $\tau$ is the observation window and $\Delta$ is the prediction
horizon. The function $f(\cdot)$ should model the transition dynamics of visuomotor
states given historical motion and egocentric perception, enabling anticipation
of visuomotor coordination under natural human motion dynamics.

% % \subsection{Predicting Visuomotor Coordination}
% \subsection{Visuomotor State Forecasting}
% \label{subsec:forecasttask}

% Given a \textit{VCR sequence}, represented as a sequence of visuomotor states
% \(
% S_{t-\tau:t} = \{S_{t-\tau}, \dots, S_t\},
% \)
% together with its corresponding egocentric video clip $E \in \mathbb{R}^{C \times T \times H \times W}$, the goal is to predict the
% future visuomotor states $\hat{S}_{t+1:t+\Delta}$ over a horizon of $\Delta$ steps. This requires modeling the temporal evolution of head pose, gaze, and upper-body joint dynamics conditioned on past kinematic and visual cues.

% Formally, we define the \textit{Visuomotor Forecasting Task} as learning a function
% \vspace{-6pt}
% \[
% \hat{S}_{t+1:t+\Delta}
%     % = f(S_{t-\Delta:t},\, E_{t-\Delta:t}),
%     = f(S_{t-\tau:t},\, E_{t-\tau:t}),
% \]
% where $\tau$ denotes the observation window and $\Delta$ is the prediction horizon. $f(\cdot)$ models the transition dynamics of visuomotor states given historical motion and egocentric perception, enabling anticipation of visuomotor coordination under natural human motion dynamics.

% Given a Visuomotor Coordination Representation (S) sequence \( S_{t-\tau:t} = \{S_t, S_{t-1}, \dots, S_{t-\tau}\} \) and its corresponding egocentric video clip \( E \in \mathbb{R}^{C \times T \times H \times W} \) , our goal is to predict the future visuomotor states \( \hat{S}_{t+1:t+\Delta} \) over a prediction horizon of \( \Delta \) steps. This task requires joint modeling of the temporal evolution of human motion, including head pose, gaze, and upper-body joint dynamics, based on past visual and kinematic observations. 

% Formally, we define the \textit{Visuomotor Forecasting Task} as learning a function:
% \[
% \hat{S}_{t+1:t+\Delta} = f(S_{t-\Delta:t}, E_{t-\Delta:t}),
% \]
% where \( f(\cdot) \) models the transition dynamics of visuomotor states given historical motion and egocentric perception, from which enables anticipation of human visuomotor coordination in dynamic environments.

\begin{figure}[t]
  \centering
   \includegraphics[width=0.9\linewidth]{figs/canon.png}
   \vspace{-12pt}
   % \caption{Visuomotor State Canonicalization Pipeline.}
    % \caption{Illustration of the canonicalization process for visuomotor states that help mitigate the effects of absolute head motion and viewpoint variations.}
    \caption{Overview of the canonicalization pipeline aligning head, gaze, and upper-body motion to the reference frame of the last observed head pose.}
   \label{fig:visuomotor-canon}
   % \vspace{-12pt}
\end{figure}

\subsection{Visuomotor State Canonicalization}
\label{subsec:canonicalization}
We canonicalize visuomotor states to provide a stable spatial reference that removes absolute head motion while preserving all relative relationships. 
Intuitively, this transformation aligns all observations to the coordinate frame of the final observed head pose, allowing the model to focus on relative motion rather than global movement. \\
Let the head pose at the final observed timestep be \(H_t=(\mathbf{p}_{\text{head},t},\,\mathbf{R}_{\text{head},t})\). We define a canonical transform \(\Phi\) that maps \(H_t\) to the origin and identity, implemented by
\[
\mathbf{R}_c=\mathbf{R}_{\text{head},t}^{\top}, \qquad 
\mathbf{p}_c=-\mathbf{R}_{\text{head},t}^{\top}\mathbf{p}_{\text{head},t}.
\]
This gives \(\Phi(H_t)=(\mathbf{0},\mathbf{I})\) and establishes a consistent reference frame.

To preserve intra-state spatial consistency, the same rigid transform is applied to all components of the visuomotor state \(S_t=\{H_t,\,\mathbf{g}_t,\,U_t\}\), yielding
\[
S_t^{c}=\Phi(S_t), \qquad 
\mathbf{g}_t^{c}=\mathbf{R}_c\mathbf{g}_t+\mathbf{p}_c, \quad
U_t^{c}=\mathbf{R}_c U_t+\mathbf{p}_c.
\]

To preserve inter-state temporal consistency across the window \(i\in[t-\tau,\,t+\Delta]\), each state is first expressed relative to \(S_t\) and then mapped to the canonical frame:
\[
S_i^{c}=T_{i\to t}(S_i)\circ S_t^{c}.
\]
This ensures that all frames remain spatially and temporally aligned, allowing the model to learn visuomotor coordination independent of viewpoint changes.

Canonicalized states are used in all experiments; for clarity, we continue to denote them as \(S_t\) in the main text. The full processing pipeline is visualized in Figure~\ref{fig:visuomotor-canon}.



% \subsection{Visuomotor State Canonicalization} 
% \label{subsec:canonicalization}
% We canonicalize kinematic data to ensure consistency across time and spatial frames. To achieve this, we standardize all motion data by defining a stable reference frame based on the final observation. Specifically, we set the head pose \( H_t = (\mathbf{p}_{\text{head},t}, \mathbf{R}_{\text{head},t}) \) in the \textit{last observed step} to a canonical state, applying the transformation \( H^c_t = \Phi(H_t) \), where \( \Phi \) normalizes the head pose by aligning its orientation to identity rotation \( \mathbf{I} \) and positioning it at the origin \( \mathbf{0} \). This transformation ensures consistency across time, allowing the model to learn visuomotor coordination independently of absolute head motion.  

% To preserve intra-state spatial consistency, the same transformation \( \Phi \) is applied to the gaze endpoint \( \mathbf{g}_t \) and upper-body joint positions \( U_t \) through \( \mathbf{g}^c_t = \Phi(\mathbf{g}_t) \) and \( U^c_t = \Phi(U_t) \). This results in \( S^c_t = \Phi(S_t)\), where all visuomotor elements remain consistent relative to the canonical head frame, ensuring the model captures meaningful coordination patterns without being affected by head motion variations.  

% To preserve inter-state temporal consistency, we extend this operation to all preceding and future kinematic states. For kinematic states \( S_i \) with \( i \in [t - \tau, t + \Delta] \), each state is first transformed relative to \( S_t \) before being mapped to the canonical frame. As a result, we have  
% \(
% S^c_i = T_{i \to t}(S_i) \circ S^c_t,
% \)
% where \( S^c_t = \Phi(S_t) \) is the canonicalized reference state. This ensures that all frames remain correctly aligned relative to each other, preserving both temporal and spatial consistency.

% This process removes absolute head motion while preserving the relative relationships between the head, gaze, and upper-body joints. It enables the model to learn visuomotor coordination independently of viewpoint variations, improving robustness and generalization. An example of this processing pipeline is shown in Fig.~\ref{fig:visuomotor-canon}. Note that \( S^c_t \) is used in the experiments; however, for simplicity, we continue using the notation \( S_t \) throughout this paper.


\subsection{Model Architecture}
\label{subsec:arch}
We first describe how we extract and fuse multimodal information to construct the conditioning feature for diffusion (Sec.~\ref{subsec:cond_feat}), followed by the diffusion-based visuomotor prediction process (Sec.~\ref{subsec:diffusion_pred}). Figure~\ref{fig:modelarch} provides an overview of our model.
\subsubsection{Conditioning Feature Extraction}
\label{subsec:cond_feat}
% \noindent \textbf{Multimodal Feature Encoding.} Given a sequence of visuomotor states \( S_{t-\tau:t} \) sampled at 10 fps, where each state \( S_t = \{H_t, G_t, U_t\} \) consists of \textit{head pose}, \textit{gaze direction}, and \textit{upper-body joints}, we project them into a latent space using learned functions: \( \mathbf{k}^{\text{head}}_t = f_h(H_t) \), \( \mathbf{k}^{\text{gaze}}_t = f_g(G_t) \), and \( \mathbf{k}^{\text{joint}}_t = f_u(U_t) \). Egocentric RGB frames \( E_{t-\tau:t} \) are sampled at 4 fps, providing complementary contextual information about the environment and task-relevant objects. A single visual embedding \( \mathbf{v} = \mathcal{F}_{\text{vis}}(E_{t-\tau:t}) \) is extracted from the sequence using a 3D ResNet backbone.

\noindent \textbf{Multimodal Feature Encoding.}  
A sequence of visuomotor states \( S_{t-\tau:t} \) is sampled at 10 fps.  
Each state \( S_t = \{ H_t, G_t, U_t \} \) contains the head pose, gaze direction, and upper body joints, which are projected into a latent space through learned functions:
\begin{equation*}
    \begin{aligned}
        % \[
        \mathbf{k}_t^{H} = f_h(H_t), \qquad 
        \mathbf{k}_t^{G} = f_g(G_t), \qquad
        \mathbf{k}_t^{U} = f_u(U_t).
        % \]
    \end{aligned}
\end{equation*}
\noindent Egocentric RGB frames \( E_{t-\tau:t} \) are sampled at 4 fps and provide visual context about the surrounding scene and task related objects.  
A 3D ResNet backbone processes the entire window \( E_{t-\tau:t} \) and produces a single visual embedding 
\(\mathbf{v} = \mathcal{F}_{\text{vis}}(E_{t-\tau:t}) \in \mathbb{R}^{128}\).

% \noindent \textbf{Multimodal Feature Encoding}  
% Given a sequence of visuomotor states \( S_{t-\tau:t} \) sampled at 10 fps, where each state  
% \( S_t = \{ H_t, G_t, U_t \} \) consists of head pose, gaze direction, and upper-body joints, we project them into a latent space using learned functions:
% \(
% \mathbf{k}_t^{H} = f_h(H_t), \quad \mathbf{k}_t^{G} = f_g(G_t), \quad \mathbf{k}_t^{U} = f_u(U_t).
% \)
% Egocentric RGB frames \( E_{t-\tau:t} \) are sampled at 4 fps, providing complementary visual cues about the environment and attended objects.
% % complementary contextual information about the environment and task-relevant objects. 
% We use a 3D ResNet backbone to extract a single visual embedding  
% \(
% \mathbf{v} = \mathcal{F}_{\text{vis}}(E_{t-\tau:t}) \in \mathbb{R}^{128}
% \)
% from them.

% \noindent \textbf{Multimodal Feature Fusion.} 
\noindent \textbf{Structured Multimodal Fusion.} We adopt a structured grouping to introduce a clearer inductive bias for visuomotor coordination. Head orientation and gaze direction jointly encode viewpoint and attentional targets, while upper-body joints contain execution-level motion cues. To preserve this structure, we form two kinematic groupings:
\begin{equation*}
    \begin{aligned}
        % \[
        \mathbf{k}^{HG}_t = \text{Concat}(\mathbf{k}^H_t, \mathbf{k}^G_t),\;
        \mathbf{k}^{HGU}_t = \text{Concat}(\mathbf{k}^H_t, \mathbf{k}^G_t, \mathbf{k}^U_t).
        % \]
    \end{aligned}
\end{equation*}
% \vspace{-12pt}
\noindent Since $\mathbf{k}^{HGU}_t$ resides in a higher-dimensional space, we apply a projection layer $f_{\text{proj}}$ to match the latent dimension expected by the denoiser. Cross-attention is applied separately to each grouping, using the visual embedding $\mathbf{v}$ as keys and values:
\begin{equation*}
    \begin{aligned}
        \mathbf{k}'^{HG}_t  = \mathcal{A}(\mathbf{k}^{HG}_t, \mathbf{v}, \mathbf{v}),\;
        \mathbf{k}'^{HGU}_t = \mathcal{A}(f_{\text{proj}}(\mathbf{k}^{HGU}_t), \mathbf{v}, \mathbf{v}).
    \end{aligned}
\end{equation*}
% \vspace{-6pt}

\noindent This decoupled design preserves the roles of head orientation and gaze direction as viewpoint and attentional cues, while integrating upper-body motion through a separate pathway. The two attended features are summed to form
\[
\mathbf{k}^{\text{fused}}_t = \mathbf{k}'^{HG}_t + \mathbf{k}'^{HGU}_t.
\]
\noindent The fused sequence is processed by a temporal self-attention encoder, which produces the conditioning vector $\mathbf{c}$ for the diffusion model. The denoiser $\mathcal{D}$ follows the temporal U-Net of \cite{chi2023diffusion} and predicts noise at each timestep.

% \noindent This decoupled design preserves the roles of head orientation and gaze direction as viewpoint and attentional cues, while integrating upper-body motion through a separate pathway. The two attended features are summed to form the fused representation:
% \(
% \mathbf{k}^{\text{fused}}_t = \mathbf{k}'^{HG}_t + \mathbf{k}'^{HGU}_t.
% \)
% \noindent A temporal self-attention layer
% % temporal Transformer encoder 
% $\mathcal{T}$ processes the fused sequence to produce a conditioning vector $\mathbf{c}$, which is fed into the denoiser $\mathcal{D}$ of the diffusion model.
% \[
% \mathbf{k}'^{HG}_t  = \mathcal{A}(\mathbf{k}^{HG}_t, \mathbf{v}, \mathbf{v}),\qquad
% \mathbf{k}'^{HGU}_t = \mathcal{A}(f_{\text{proj}}(\mathbf{k}^{HGU}_t), \mathbf{v}, \mathbf{v}).
% \]
% While egocentric frames always contain cues directly related to head and gaze orientation, their relevance to full visuomotor coordination is uncertain due to partial occlusions and viewpoint limitations. To mitigate this, instead of using a single kinematic representation, we construct two separate kinematic representations: 

% one capturing head and gaze features, defined as \( \mathbf{k}^{\text{hg}}_t = \text{Concat}(\mathbf{k}^{\text{head}}_t, \mathbf{k}^{\text{gaze}}_t) \), and another incorporating full-body motion as \( \mathbf{k}^{\text{hga}}_t = \text{Concat}(\mathbf{k}^{\text{head}}_t, \mathbf{k}^{\text{gaze}}_t, \mathbf{k}^{\text{arm}}_t) \). 

% \noindent We apply cross-attention separately to \( \mathbf{k}^{\text{hg}}_t \), which captures viewpoint and attentional dynamics, and to \( \mathbf{k}^{\text{hga}}_t \), which additionally includes upper-body motion cues. This structured fusion allows the model to selectively incorporate spatial and attentional signals while maintaining robustness to missing or ambiguous visual information. Formally, we compute:
% \vspace{-6pt}
% \begin{equation*}
%     \begin{aligned}
%         \mathbf{k}^{\prime \text{hg}}_t &= \mathcal{A}(\mathbf{k}^{\text{hg}}_t, \mathbf{v}, \mathbf{v}), \quad 
%         \mathbf{k}^{\prime \text{hga}}_t &= \mathcal{A}(f_{\text{proj}}(\mathbf{k}^{\text{hga}}_t), \mathbf{v}, \mathbf{v}).
%     \end{aligned}
% \end{equation*}
% \vspace{-12pt}

% \noindent The final fused representation is obtained by summing the attended features:  
% \( \mathbf{k}_t^{\text{fused}} = \mathbf{k}^{\prime \text{hg}}_t + \mathbf{k}^{\prime \text{hga}}_t \), which is then passed to a Transformer-based temporal encoder \(\mathcal{T}\) for sequential modeling. The output is flattened into a single conditioning feature \( \mathbf{c} \), which is used as input to the denoiser \(\mathcal{D}\).
% \vspace{-6pt}

% \subsection{Invariant Processing.} At both training and inference stages, kinematic data are canonicalized for consistency. The head pose in the final observation frame is set to a fixed state, aligning its orientation to identity rotation and positioning it at the origin. To maintain spatial consistency, gaze direction and upper-body joints in the same frame are transformed accordingly. All preceding and future kinematic states are adjusted relative to this reference frame, ensuring a unified coordinate system for model inputs and predictions. {\color{red}TODO}

% By establishing a stable reference frame and applying consistent transformations across time, this process ensures that the model learns visuomotor coordination without being affected by absolute head motion. The proposed canonicalization not only maintains spatial and temporal consistency but also preserves both inter-state and inner-state relationships. This enables the model to focus on predicting meaningful coordination dynamics while ensuring robustness to variations in head movement.

% The full transformation consists of two steps:  
% \begin{itemize}
%     \item \( T_{i \to t}(S_i) = (\mathbf{R}_{\text{head},t}^{-1} \mathbf{R}_{\text{head},i}, \mathbf{R}_{\text{head},t}^{-1} (\mathbf{p}_{\text{head},i} - \mathbf{p}_{\text{head},t})) \)
%     \item \( S^c_i = \Phi(T_{i \to t}(S_i))\)
% \end{itemize}


% This operation to all preceding and future kinematic states to preserve inter-state consistency, ensuring that relative positions between consecutive frames remain unchanged. Simultaneously, it maintains inner-state consistency, preserving the spatial relationships between the head, gaze, and upper-body joints within each frame.  


% By applying these transformations sequentially, the entire sequence is represented in a unified reference frame, eliminating the influence of head motion while preserving spatial relationships between the head, gaze, and upper-body joints. This allows the model to focus on learning visuomotor coordination dynamics without being affected by absolute head movements.

% At both training and inference stages, we canonicalize kinematic data to ensure consistency across time and spatial frames. To achieve this, we standardize all motion data by defining a stable reference frame based on the final observation. 
% Specifically, we set the head pose \( H_t = (\mathbf{p}_{\text{head},t}, \mathbf{R}_{\text{head},t}) \) in the \textit{last observed step} to a canonical state, applying the transformation: \(H^c_t = \Phi(H_t)\), where \( \Phi \) normalizes the head pose by aligning its orientation to identity rotation \(\mathbf{I}\) and positioning it at the origin \(\mathbf{0}\). This transformation ensures consistency across time, allowing the model to learn visuomotor coordination independently of absolute head motion. 

% To preserve spatial relationships, the same transformation \( \Phi \) is applied to the gaze endpoint \( \mathbf{g}_t \) and upper-body joint positions \( U_t \) through \(\mathbf{g}^c_t = \Phi(\mathbf{g}_t), \quad U^c_t = \Phi(U_t)\). Now we have \(S^c_t\), in which all visuomotor elements remain consistent relative to the canonical head frame, ensuring the model captures meaningful coordination patterns without being affected by head motion variations.

% This operation is applied to all preceding and future kinematic states to preserve inter-state consistency, ensuring that relative positions between consecutive frames remain unchanged. Simultaneously, it maintains inner-state consistency, preserving the spatial relationships between the head, gaze, and upper-body joints within each frame.

% From this point, for kinematic states \( S_i \) with \( i \in [t - \tau, t + \Delta] \), it must be first transformed relative to \( S_t \) before being mapped to the canonical frame. For each step, the full transformation is decomposed into two parts:
% \begin{itemize}
%     \item Computing the relative transformation from \( i \) to \( t \):
%     \[
%     T_{i \to t}(S_i) = (\mathbf{R}_{\text{head},t}^{-1} \mathbf{R}_{\text{head},i}, \quad \mathbf{R}_{\text{head},t}^{-1} (\mathbf{p}_{\text{head},i} - \mathbf{p}_{\text{head},t}))
%     \]
%     This step expresses the kinematic state at frame \( i \) in the local coordinate system of frame \( t \), ensuring that relative spatial relationships between frames are preserved.

%     \item Applying the transformation from \( t \) to the canonical frame:
%     \[
%     S^c_i = \Phi(T_{i \to t}(S_i))
%     \]
%     where \( \Phi \) is the transformation function that maps the frame-aligned state to the canonical space. This ensures that all kinematic states are expressed in a unified reference frame while maintaining both inter-state and inner-state consistency.
% \end{itemize}

% By applying these transformations sequentially, we ensure that the entire sequence is represented in a unified reference frame, eliminating the influence of head motion while preserving spatial relationships between the head, gaze, and upper-body joints. This allows the model to focus on learning visuomotor coordination dynamics without being affected by absolute head movements.



% \begin{itemize}
%     \item Rotation Alignment: The head orientation is transformed to the identity by applying \( \mathbf{R}_{\text{head},t}^{-1} \).
%     \item Position Normalization: The head position is translated to the origin by subtracting \( \mathbf{p}_{\text{head},t} \).
% \end{itemize}

% Applying this transformation to any kinematic point \( \mathbf{p} \), such as gaze \( G_t \) or upper-body joints \( U_t \), results in:

% \[
% \tilde{\mathbf{p}} = \mathbf{R}_{\text{head},t}^{-1} (\mathbf{p} - \mathbf{p}_{\text{head},t}).
% \]

% This transformation ensures that all motion data remains consistent within a unified reference frame, allowing the model to learn **visuomotor coordination** independently of absolute head motion.


% To maintain spatial consistency, the gaze component \( G_t \) and upper-body joints \( U_t \) are transformed accordingly. The translation between 

% including shoulders, elbows, and wrists, are expressed relative to the transformed head frame.  

% Furthermore, all preceding and future kinematic states are transformed into this unified coordinate system. Given an observation sequence \( S_{t-\tau:t} = \{ S_t, S_{t-1}, \dots, S_{t-\tau} \} \), we align all states within a stable reference frame, ensuring model inputs and predictions remain invariant to camera motion and egocentric viewpoint shifts. The transformation is given by:
% \[
% H a^p_{t:t+h} = [(T^W_{F_t})^{-1} T^W_{F_i} p_i^{F_i}] \quad \text{for } i \in [t, t+1, \dots, t+h]
% \]
% This transformation eliminates viewpoint variations, allowing the model to focus on relative motion patterns rather than absolute spatial shifts.  
% By creating a unified reference frame, the model can learn visuomotor coordination patterns without being affected by variations in head pose or observation perspective.

% \subsection{Invariant Processing}  
% At both training and inference stages, we canonicalize kinematic data to ensure consistency across time and spatial frames. To achieve this, we standardize all motion data by defining a stable reference frame based on the final head orientation observation \( \mathbf{R}_{\text{head}}) \).  

% Specifically, the head pose \( H = (\mathbf{p}_{\text{head}}, \mathbf{R}_{\text{head}}) \) in the last observed frame is fixed to a canonical state by aligning its orientation to the identity rotation \( \mathbf{R}_{\text{head}} = \mathbf{I} \) and positioning it at the origin \( \mathbf{p}_{\text{head}} = \mathbf{0} \). This transformation eliminates viewpoint variations, allowing the model to focus on relative motion patterns rather than absolute spatial shifts.  

% To maintain spatial consistency, the gaze component \( G \), represented by the **gaze endpoint** \( g \), and upper-body joints \( U \) are transformed accordingly. The upper-body joint positions:
% \[
% U = \{\mathbf{j}_i \in \mathbb{R}^3 \mid i = 1, \dots, 6\}
% \]
% including shoulders, elbows, and wrists, are expressed relative to the transformed head frame.  

% Furthermore, all preceding and future kinematic states are transformed into this unified coordinate system. Given a **Visuomotor Coordination Representation (VCR) sequence** \( S_{t-\tau:t} = \{ S_t, S_{t-1}, \dots, S_{t-\tau} \} \), we align all states within a stable reference frame, ensuring **model inputs and predictions** remain invariant to camera motion and egocentric viewpoint shifts. The transformation is given by:
% \[
% H a^p_{t:t+h} = [(T^W_{F_t})^{-1} T^W_{F_i} p_i^{F_i}] \quad \text{for } i \in [t, t+1, \dots, t+h]
% \]

% By creating a unified reference frame, the model can learn visuomotor coordination patterns without being affected by variations in head pose or observation perspective.

% \subsection{Invariant Processing}  
% At both training and inference stages, we canonicalize kinematic data to ensure consistency across time and spatial frames. To achieve this, we standardize all motion data by defining a stable reference frame based on the final observation.  

% Specifically, the head pose in the last observed frame is fixed to a canonical state, aligning its orientation to an identity rotation and positioning it at the origin. This transformation eliminates viewpoint variations, allowing the model to focus on relative motion patterns rather than absolute spatial shifts.  

% To maintain spatial consistency, gaze direction and upper-body joints in the same frame are transformed accordingly. Their positions and orientations are re-expressed relative to the canonical head pose, ensuring that all movement data remains coherent under this reference frame.  

% Furthermore, all preceding and future kinematic states are transformed into this unified coordinate system. This adjustment ensures that both model inputs and predictions are invariant to camera motion and egocentric viewpoint shifts. As a result, the model learns visuomotor coordination patterns without being affected by variations in head pose or observation perspective.



% {\color{red}\subsubsection{Diffusion-Based Visuomotor Prediction}}
\subsubsection{Diffusion-Based Visuomotor Prediction}
\label{subsec:diffusion_pred}
We follow \cite{chi2023diffusion} to formulate visuomotor forecasting as a denoising diffusion process, where the model learns to iteratively refine a noisy sequence into a future trajectory. 

\noindent \textbf{Forward Diffusion Process.}  
Following the standard denoising diffusion probabilistic model (DDPM) \cite{ho2020denoising}, we define the forward process as a Markovian sequence that progressively adds Gaussian noise to the ground-truth future visuomotor states \( S_{t+1:T} \):
\vspace{-6pt}
\begin{equation*}
    q(S_t | S_0) = \mathcal{N}(S_t; \sqrt{\bar{\alpha}_t} S_0, (1 - \bar{\alpha}_t) \mathbf{I})
\end{equation*}
where \( \bar{\alpha}_t \) is a pre-defined noise schedule. This process converts the original data distribution into an isotropic Gaussian in the latent space.

\noindent \textbf{Reverse Denoising Process.}  
The model learns to iteratively denoise the corrupted future states using a neural network parameterized by \( \theta \). The reverse process is defined as:
\vspace{-6pt}
\begin{equation*}
    p_{\theta}(S_{t-1} | S_t, \mathbf{c}) = \mathcal{N}(S_{t-1}; \mu_{\theta}(S_t, t, \mathbf{c}), \sigma_{\theta}^2 \mathbf{I})
\end{equation*}
where \( \mu_{\theta} \) is the predicted mean, \( \sigma_{\theta}^2 \) is the variance, and the conditioning feature \( \mathbf{c} \) remains constant throughout the denoising process.

\noindent The model is trained using a standard denoising loss:
\begin{equation*}
    \mathcal{L} = \mathbb{E}_{S_0, t, \boldsymbol{\epsilon}} \left[ || \boldsymbol{\epsilon} - \epsilon_{\theta}(S_t, t, \mathbf{c}) ||^2 \right]
\end{equation*}
where \( \epsilon_{\theta} \) represents the noise prediction network.

\noindent At inference time, we sample future visuomotor trajectories by iteratively applying the learned reverse process, starting from standard Gaussian noise.
% starting from a Gaussian prior.


\begin{figure}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   % \includegraphics[width=1.0\linewidth]{figs/model_draft.png}
   \includegraphics[width=0.7\linewidth]{figs/new_arch.png}
    \caption{
    \textbf{Model architecture.} Kinematic features $f_h, f_g, f_u$ and a visual embedding $\mathbf{v}$ are fused by cross-attention. The fused sequence is processed by a temporal self-attention encoder, followed by a diffusion denoiser to forecast future visuomotor kinematics.
    % Model architecture. Kinematic features $f_h, f_g, f_u$ and a visual embedding $\mathbf{v}$ are fused through two cross-attention pathways corresponding to head--gaze and head--gaze--upper-body groupings. The fused sequence is processed by a temporal encoder and a diffusion denoiser to predict future kinematics.
    }
    % \vspace{-12pt}
   \label{fig:modelarch}
\end{figure}
% \vspace{-6pt}

% \subsection{Canonicalized Visuomotor Coordination}
% {\color{red}Inspired by Egoallo, I'm trying to normalize the head-gaze coordination further (ongoing now)}

% \subsection{Future Motion Description}

% \noindent \textbf{Nymeria Subset} \cite{ma2024nymeria}, in contrast, offers a different perspective by capturing long-horizon, in-the-wild human activities. While these activities still engage the motor system, the integration between visual and motor processes tends to be less precise and more adaptable to dynamic environments. Nymeria pairs egocentric video data from Aria glasses with full-body motion data from XSens motion capture suits \cite{xsenses}. With over 300 hours of egocentric footage, Nymeria is well-suited for assessing the generalizability of our approach to more spontaneous, daily-life scenarios. Similar to EgoExo4D, we also select a subset of activities from Nymeria for evaluation. This subset results in xxxxx training samples and xxxx testing samples from Nymeria. Specific task categories are included and excluded from our model training and the details can be found in the supplementary materials.

==> sec/4_experiment.tex <==
\section{Experiments}
\label{sec:experiments}
We conduct extensive experiments to evaluate our predictive visuomotor learning framework. We first introduce the datasets used in our study (Sec.~\ref{subsec:dataset}), followed by the evaluation metrics (Sec.~\ref{subsec:metrics}) used to assess prediction accuracy. We then present the baselines for comparison (Sec.~\ref{subsec:baseline}) and analyze the impact of different model components through ablation studies (Sec.~\ref{subsec:abla}). Finally, we provide both quantitative (Sec.~\ref{subsec:quanti}) results and qualitative (Sec.~\ref{subsec:quali}) to demonstrate the effectiveness of our approach.  

% {\color{blue}\subsection{Datasets and Metrics}}
% \subsection{Datasets and Metrics}
\subsection{Datasets}
\label{subsec:dataset}
% \noindent \textbf{EgoExo4D} \cite{grauman2024ego} is a large-scale multimodal egocentric-exocentric video dataset collected by Meta. It utilizes Aria glasses \cite{engel2023project} alongside four GoPro cameras to capture aligned first-person and third-person views of skilled activities across more than 130 scene contexts, totaling approximately 88 hours of egocentric footage. While the dataset encompasses a diverse range of activities, not all are equally suited for studying visuomotor coordination. We select a subset of activities where participants manipulate objects and navigate their environment in ways that naturally integrate visual attention with motor actions. The selected scenarios include Basketball, Cooking, Bike Fixing, and Health related task, resulting in 23,372 training samples and 5,126 testing samples, with a total duration of approximately 15.8 hours. 


\noindent \textbf{EgoExo4D} \cite{grauman2024ego} is a large-scale multimodal egocentric–exocentric video dataset collected by the Ego4D Consortium. It utilizes Aria glasses \cite{engel2023project} alongside four GoPro cameras to capture aligned first-person (egocentric) and third-person (exocentric) views of skilled activities across more than 130 scene contexts, totaling approximately 88 hours of egocentric footage.
The dataset provides head pose and gaze annotations computed by Meta’s Multimodal Perception Service (MPS), ensuring accurate SLAM-based pose estimation. Additionally, full-body 3D joint positions are annotated from the exocentric videos.

While EgoExo4D encompasses a diverse range of activities, not all are equally suited for studying visuomotor coordination. We select a subset of activities where participants manipulate objects and engage in visually guided motor behaviors. The selected scenarios include Basketball, Cooking, Bike Fixing, and Health-related tasks, resulting in 23,372 training samples and 5,126 testing samples, with a total duration of approximately 15.8 hours.
% We focus on upper-body dynamics because these joints form the core visuomotor loop, and our selected activities involve minimal lower-body locomotion. 
Detailed information about the data cleaning pipeline and per-class statistical distribution is provided in the supplementary materials.

% We focus on upper-body dynamics for two reasons. First, our definition of
% visuomotor coordination centers on head pose, gaze behavior, and arm
% motion, which form the primary closed-loop pathway for visually guided
% manipulation. Including lower-body joints would introduce variation that
% is largely irrelevant to this coordination loop. Second, the EgoExo4D
% recording setup restricts large-scale locomotion—the actor is surrounded
% by four synchronized exocentric cameras—so lower-body movement is limited
% and often poorly captured. Focusing on the upper body therefore yields a
% cleaner and more reliable signal for visuomotor forecasting.

% Sec.~\ref{sec:dataclean} of our supplementary materials.

% % \subsection{Metrics}
% \noindent \textbf{Metrics.} Predicting Visuomotor Coordination is inherently challenging due to the need for accurate multi-modal motion forecasting, including head orientation, gaze behavior, and upper-body joint dynamics. Unlike standard motion prediction tasks, this setting requires maintaining spatiotemporal coherence across different components of the coordination system while ensuring that the predicted movement remains both biomechanically plausible and semantically meaningful over future time horizons. 

% To comprehensively evaluate the forecasting results of VCR, we employ four key metrics that capture different aspects of forecasting accuracy: (1) MPJPE quantifies the mean per-joint position error (in mm) for all body joints except head rotation. It evaluates absolute spatial accuracy, which is crucial as small errors can accumulate over long-horizon forecasting. (2) PA-MPJPE assesses structural consistency by applying Procrustes alignment before computing the joint position error. It helps evaluate whether the relative structure of the predicted VCR remains coherent, which reflects an important goal of our task. (3) H-MPJPE focuses on hand movement accuracy, isolating the mean per-joint position error for hand joints per its particularly challenging nature. (4) MPJAE measures head rotation error (degrees) to evaluate the accuracy of predicted head orientation. 

% \noindent \textbf{Metrics.} Predicting Visuomotor Coordination requires forecasting multi-modal motion, including head orientation, gaze behavior, and upper-body joint dynamics. Unlike standard motion prediction tasks, this setting demands \textbf{spatiotemporal consistency} across components while ensuring \textbf{kinematically plausible} movements and \textbf{alignment with natural visuomotor patterns} over extended time horizons.  

% \noindent To comprehensively evaluate VCR forecasting, we employ four key metrics, each capturing a distinct aspect of prediction accuracy. All metrics are computed over 10 future timesteps at 10fps and averaged accordingly: 
% \begin{itemize}
%     \item \textbf{MPJPE} (mm) measures the mean per-joint position error for all translation components, including head position, gaze ray endpoint, and all upper-body joints. It provides a direct evaluation of absolute spatial accuracy while indirectly reflecting motion consistency over time.  
%     \item \textbf{PA-MPJPE} (mm) assesses structural consistency by applying Procrustes alignment before computing position errors, ensuring that the relative spatial relationships between the head, gaze, and upper-body joints remain stable throughout the forecast. Unlike MPJPE, PA-MPJPE is computed separately at each step and averaged over 10 steps, capturing long-term coherence.  
%     \item \textbf{H-MPJPE} (mm) focuses on hand movement accuracy, isolating the mean per-joint position error for hand joints due to their inherently high complexity.   
%     \item \textbf{MAE} (degrees) measures head rotation error, evaluating the deviation of predicted head orientation from the ground truth.  

% \end{itemize}
% Together, these metrics assess spatiotemporal consistency (MPJPE, PA-MPJPE), kinematic plausibility (PA-MPJPE), and alignment with natural visuomotor patterns (MPJPE, PA-MPJPE, H-MPJPE, MAE).

% \subsection{Evaluation Metrics}

% To comprehensively evaluate our Predictive Visuomotor Learning task, we adopt a diverse set of metrics that assess \textit{structural consistency}, \textit{position errors}, and \textit{orientation accuracy}. Unlike standard motion forecasting tasks, our evaluation is designed to capture the coordination and plausibility of predicted visuomotor behaviors rather than just positional accuracy.
% \begin{itemize}
%     % \item \textbf{PA-MPJPE} (Procrustes-Aligned Mean Per Joint Position Error) measures the structural consistency of the predicted body pose. Unlike MPJPE, PA-MPJPE aligns the predicted and ground-truth poses via a rigid transformation, ensuring that the error primarily reflects internal joint structure deviations rather than global displacement.
%     \item \textbf{PA-MPJPE} (mm) assesses structural consistency by applying Procrustes alignment before computing position errors, ensuring that the relative spatial relationships between the head, gaze, and upper-body joints remain stable throughout the forecast. Unlike MPJPE, PA-MPJPE is computed separately at each step and averaged over 10 steps, capturing long-term coherence.  

    % \item \textbf{MPJPE} (mm) measures the mean per-joint position error for all translation components, including head position, gaze ray endpoint, and all upper-body joints. It provides a direct evaluation of absolute spatial accuracy while indirectly reflecting motion consistency over time.  
    % \item \textbf{PA-MPJPE} (mm) assesses structural consistency by applying Procrustes alignment before computing position errors, ensuring that the relative spatial relationships between the head, gaze, and upper-body joints remain stable throughout the forecast. Unlike MPJPE, PA-MPJPE is computed separately at each step and averaged over 10 steps, capturing long-term coherence.  
    % \item \textbf{H-MPJPE} (mm) focuses on hand movement accuracy, isolating the mean per-joint position error for hand joints due to their inherently high complexity.   
    % \item \textbf{MAE} (degrees) measures head rotation error, evaluating the deviation of predicted head orientation from the ground truth.  

% \end{itemize}
% Together, these metrics assess spatiotemporal consistency (MPJPE, PA-MPJPE), kinematic plausibility (PA-MPJPE), and alignment with natural visuomotor patterns (MPJPE, PA-MPJPE, H-MPJPE, MAE).

\subsection{Evaluation Metrics}
\label{subsec:metrics}

We evaluate our predictive visuomotor model using metrics that capture structural consistency, positional accuracy, and orientation alignment. All metrics are computed over the visuomotor state \( S = \{H, G, U\} \), as defined in Sec.~\ref{subsec:vcr}.

\noindent\textbf{Structural Consistency.} 
PA-MPJPE (mm) measures the structural accuracy of the predicted visuomotor state. The metric aligns predictions to the ground truth via a rigid transformation, ensuring that errors reflect deviations in internal joint structure rather than global motion. PA-MPJPE is computed over \( \{\mathbf{p}_{head}, G, U\} \).

\noindent\textbf{Positional Accuracy.} 
We report Euclidean position errors for key components of the visuomotor state. Head, gaze, and hand position errors correspond to \( \mathbf{p}_{head} \), \( G \), and the wrist joints \( \mathbf{j}_i \) for \( i \in \{5, 6\} \), respectively (a subset of \( U \)).

\noindent\textbf{Orientation Accuracy.} 
Head orientation accuracy is measured using Head Rotation Error (HRE, degrees), defined as the angular difference between predicted and ground-truth head rotations.

\subsection{Implementation Details}
The model is implemented in PyTorch and trained for 400 epochs on a single H100 GPU with a batch size of 384. We use AdamW with a learning rate of $5\times 10^{-4}$. The visual encoder is initialized from Kinetics-400, while the transformer layers and diffusion modules are trained from scratch. Inference requires 478.7±13.4 ms per sample with 100 DDPM steps on a single RTX 4090.


% \noindent\textbf{Orientation Accuracy.} We evaluate the accuracy of head rotation and gaze direction to measure their alignment and predictive consistency.
% \begin{itemize}
%     \item \textbf{Head Rotation Error (HRE)} (degree) measures the angular deviation between the predicted and ground-truth head orientations.
%     \item \textbf{Gaze Relative Angular Error (GRAE)} (degree) quantifies the alignment between the predicted gaze direction and predicted head orientation:
%     \begin{equation*}
%     \theta_{\text{GRAE}} = \arccos \left( \frac{\mathbf{v}_{\text{head}} \cdot \mathbf{v}_{\text{gaze}}}{\|\mathbf{v}_{\text{head}}\| \|\mathbf{v}_{\text{gaze}}\|} \right)
%     \end{equation*}
%     where the predicted gaze and head directions are computed as:
%     \begin{equation*}
%     \mathbf{v}_{\text{gaze}} = \frac{G - \mathbf{p}_{head}}{\| G - \mathbf{p}_{head} \|}, \quad
%     \mathbf{v}_{\text{head}} = \mathbf{R}_{head} \mathbf{v}_0
%     \end{equation*}
%     where \( \mathbf{v}_0 \) represents the canonical forward direction of the head in its local coordinate frame.
% \end{itemize}

% {\color{blue}\subsection{Baselines}}
\subsection{Baselines}
\label{subsec:baseline}
% Since we are the first to address the visual-motor descriptor forecasting problem, there are no pre-existing baselines directly comparable. 
% We include two naive interpolate baselines that derive simple forecasting results from observable sequences, two 
% To evaluate the effectiveness of our method, we compare it against two naïve interpolate baselines and three learning-based methods, including a standard Diffusion Policy model. Note that our work is concurrent with EgoCast\cite{escobar2025egocast}, however we cannot compare with their method due to accessble to the code. 
% To evaluate the effectiveness of our method, we compare it against two naïve interpolation baselines and three learning-based methods, including a standard Diffusion Policy model. Our work is concurrent with EgoCast~\cite{escobar2025egocast}; however, we are unable to provide a direct comparison due to the unavailability of their code.
% To evaluate the effectiveness of our method, we compare it against two naïve interpolation baselines and three learning-based methods, including a standard Diffusion Policy model.\footnote{Our work is concurrent with EgoCast~\cite{escobar2025egocast} and EgoAgent~\cite{chen2025acquisition}, but a direct comparison is not possible due to differences in task settings and the lack of publicly available code at the time of writing.}
% To evaluate the effectiveness of our method, we compare it against two naïve interpolation baselines and three learning-based methods, including a standard Diffusion Policy model.\footnote{Our work is concurrent with EgoCast~\cite{escobar2025egocast} and EgoAgent~\cite{chen2025acquisition}, but a direct comparison is not feasible due to differences in task definitions and input modalities, as well as the lack of publicly available implementations at the time of writing.}

% To evaluate the effectiveness of our method, we compare it against two naïve interpolation baselines and two learning-based methods, including a Diffusion Policy model.
To evaluate the effectiveness of our method, we compare it against two heuristic baselines and three categories of learning-based predictors:
% \footnote{Our work is concurrent with EgoCast~\cite{escobar2025egocast} and EgoAgent~\cite{chen2025acquisition}, but a direct comparison is not feasible due to differences in task definitions and input modalities, as well as the lack of publicly available implementations at the time of writing.}


\begin{itemize}
    \item \textbf{Constant Pose}: 
    Assumes no future motion by directly copying the last observed visuomotor state for all future time steps. This serves as a lower bound representing a scenario without predictive modeling.
    % assumes no future motion, directly copying the last observed visuomotor state for all future time steps. It serves as a lower bound, representing a scenario without predictive modeling.
    
    \item \textbf{Constant Velocity}: 
    % performs first-order linear extrapolation using the most recent state transition. This simple heuristic provides a basic estimate of future motion dynamics.
    Performs first-order linear extrapolation using the most recent state transition to provide a basic estimate of future motion dynamics.
    \item \textbf{Transformer-Based Model}: We evaluate two Transformer variants to assess the impact of architectural design. 
    (1) An \emph{encoder-only} model, where upper-body pose trajectories and ResNet18 visual embeddings are fed into a 3-layer Transformer encoder followed by an MLP regression head for parallel sequence prediction. 
    (2) A \emph{decoder-based} model that conditions each predicted timestep on learned decoder queries, using a Transformer decoder with cross-attention to past observations. 
    % This comparison evaluates both encoder-only and encoder–decoder formulations commonly used in motion forecasting.

    % \item \textbf{Transformer Encoder + MLP}: a standard Transformer-based sequence-to-sequence predictor. We concatenate upper-body pose trajectories with ResNet18 image embeddings and feed them into a 3-layer Transformer encoder followed by an MLP regression head to produce future visuomotor states.
    
    % \item \textbf{Transformer Decoder + MLP}: a stronger baseline that conditions each output timestep on previous predictions using a Transformer decoder with causal masking. This architecture is widely used in motion and time-series forecasting tasks and provides an autoregressive alternative to the encoder-only model.

    % \item \textbf{Autoregressive Head}: a variant of the Transformer encoder baseline where the future sequence is predicted step-by-step using an autoregressive output head. At each timestep, the model feeds its previous prediction back into the regression head while keeping the Transformer encoder frozen as a parallel feature extractor. 
    \item \textbf{Autoregressive Transformer}: A variant where the future sequence is predicted step-by-step. At each timestep, the model feeds its previous prediction back into the regression head while utilizing the Transformer encoder as a parallel feature extractor.
    
    \item \textbf{Diffusion Policy (CNN-Based) \cite{chi2023diffusion}}: 
    % models future motion as a denoising diffusion process. We adapt the method by extracting egocentric visual features via ResNet18 and concatenating them with raw visuomotor observations. The resulting flattened sequence is used as conditioning input to a U-Net denoiser that refines noisy motion trajectories.
    Models future motion as a denoising diffusion process. We adapt this method by extracting egocentric visual features via ResNet18 and concatenating them with raw visuomotor observations as input to a U-Net denoiser that refines noisy motion trajectories.

    % \item \textbf{Constant Pose}: assumes no future motion, directly copying the last observed visuomotor state for all future time steps. It serves as a lower bound, representing a scenario where no predictive modeling is performed.
    % \item \textbf{Constant Velocity}: estimates future motion using first-order linear extrapolation, assuming a constant velocity based on the last observed state transition. It provides a simple motion forecasting heuristic.
    % % \item \textbf{siMLPe\cite{guo2023back}}: is an MLP-based motion forecasting model that captures spatiotemporal dependencies using a lightweight and efficient architecture. It applies structured modeling to human motion sequences while maintaining low computational overhead.
    % \item \textbf{Transformer Model}: is a standard Transformer-based sequence-to-sequence predictor that models motion evolution through self-attention. We concatenate pose sequences with visual embeddings extracted from ResNet18 and feed them into a 3-layer Transformer encoder, followed by a regression head to predict future visuomotor states. 
    % \item \textbf{Diffusion Policy (CNN-Based) \cite{chi2023diffusion}}: formulates motion prediction as a denoising diffusion process, where a neural network iteratively refines a noisy motion sequence into a plausible future trajectory. We apply this framework to our setting by extracting egocentric frame features using a pre-trained ResNet18, concatenating them with raw visuomotor observations, and flattening the resulting feature representation to condition a U-Net denoiser. 
\end{itemize}

\begin{table*}[h!]
\centering
\footnotesize 
{\setlength{\tabcolsep}{6pt}
\begin{tabular}{ccccccc}
% \hline
\toprule
\textbf{Category} & \textbf{Methods} & \textbf{PA-MPJPE} & \textbf{Head Pos.} & \textbf{Gaze Pos.} & \textbf{Hand Pos.} & \textbf{Head Rot.} \\ 
\midrule

\multirow{2}{*}{Heuristic} 
% & \textsc{Constant Pose} & 68 & 184 & 193 & 274 & 16.7 \\ 
% & \textsc{Constant Velocity} & 109 & 161 & 201 & 436 & 18.5 \\ 
& Constant Pose & 68 & 184 & 193 & 274 & 16.7 \\ 
& Constant Velocity & 109 & 161 & 201 & 436 & 18.5 \\ 
\hline

\multirow{3}{*}{Transformer-based} 
& Transformer Encoder + MLP & 65 & 119 & 135 & 211 & 13.8 \\
& Transformer Decoder & 60 & 119 & 137 & 204 & 14.4 \\
& Autoregressive Transformer & 71 & 149 & 165 & 239 & 16.8 \\
\hline

\multirow{2}{*}{Diffusion-based} 
& Diffusion Policy-CNN \cite{chi2023diffusion} & 64 & 112 & 132 & 208 & 13.9 \\
& \cellcolor{green!20}\textbf{Ours} 
& \cellcolor{green!20}\textbf{59} $\pm{\scriptstyle0.36}$ 
& \cellcolor{green!20}\textbf{106} $\pm{\scriptstyle0.33}$ 
& \cellcolor{green!20}\textbf{124} $\pm{\scriptstyle0.44}$ 
& \cellcolor{green!20}\textbf{188} $\pm{\scriptstyle0.76}$ 
& \cellcolor{green!20}\textbf{13.2} $\pm{\scriptstyle0.08}$ \\
\bottomrule

\end{tabular}
}
\caption{
\textbf{Quantitative Comparison of Forecasting models on EgoExo4D.}
We group methods into heuristic baselines, transformer-based predictors (including both a transformer decoder and an autoregressive variant), and diffusion-based models. 
Metrics report 3D prediction error for pose-aligned MPJPE, head position, 3D gaze endpoint, hand position, and head rotation (lower is better). 
Our method achieves the lowest error across all visuomotor components.
}
\label{tab:baseline}
\end{table*}


% \begin{table*}[h!]
% \centering
% \footnotesize 
% {\setlength{\tabcolsep}{8pt} % Adjust column spacing
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%          Methods & PA-MPJPE & Head Pos. & Gaze Pos. & Hand Pos. & Head Rot. \\ \hline
%         \textsc{Constant Pose} &  68 &  184 & 193 & 274 & 16.7 \\ 
%         \textsc{Constant Velocity} &  109 & 161 & 201 & 436  &  18.5 \\ 
%         Transformer Encoder + MLP &  65 & 119 & 135 & 211 & 13.8 \\
%         Transformer Decoder + MLP &  60 & 119 & 137 & 204 & 14.4 \\
%         Diffusion Policy-CNN \cite{chi2023diffusion} & 64  & 112 & 132 & 208 & 13.9 \\
%         \cellcolor{green!20}\textbf{Ours} & \cellcolor{green!20}\textbf{59} $\pm {\scriptstyle0.36}$ & \cellcolor{green!20}\textbf{106} $\pm {\scriptstyle0.33}$ & \cellcolor{green!20}\textbf{124} $\pm {\scriptstyle0.44}$ & \cellcolor{green!20}\textbf{188} $\pm {\scriptstyle0.76}$ & \cellcolor{green!20}\textbf{13.2} $\pm {\scriptstyle 0.08}$ \\ \hline
%     \end{tabular}}
%     % \vspace{-6pt}
%     % \caption{\textbf{Quantitative comparison of our method against baselines.} Lower values indicate better performance.
%      \caption{\textbf{Quantitative comparison of our approach with baseline forecasting models on EgoExo4D.} Metrics reflect 3D prediction error for pose-aligned MPJPE, head position, 3D gaze endpoint, hand position, and head rotation (lower is better). Our method achieves the best performance across all visuomotor components.
%     % {\color{red}TODO: add results on top 5\% hardest sample to validate simple performance. adding simple viz if have time.}
%     }
%     % \vspace{-6pt}
% \label{tab:baseline}
% \end{table*}

% \renewcommand{\arraystretch}{1.1} 
% \begin{table*}[h!]
% \centering
% \footnotesize 
% {\setlength{\tabcolsep}{8pt} % Default value: 6pt
% % \renewcommand{\arraystretch}{1} % Default value: 1
%     \begin{tabular}{c|c|c|c|c|c}
%         \hline
%         % \multicolumn{1}{c|}{\multirow{2}{*}{}} &\multicolumn{2}{c|}{Head Pose} &\multicolumn{1}{c|}{Gaze Pose} &\multicolumn{3}{c|}{Arm Pose} & \multicolumn{1}{|c}{}\\ 
%         % \cline{2-8}
%         % \hline
%          \multirow{1}{*}{} & Methods & PA-MPJPE , \% & MPJPE , \% & H-MPJPE , \% & MAE , \% \\ \hline
%         \multirow{2}{*}{\centering Naïve Interpolate} & \textsc{Constant Pose} &  68.3, + 16.6 & 215 , + 59.3 & 274 , + 44.9 & 16.7 , + 25.6\       \\ 
%         \multirow{2}{*}{} & \textsc{Constant Velocity} &  109, + 84.7 & 264 , + 95.6 & 436 , + 131  &  18.5 , + 39.1 \\
%         \multirow{2}{*}{\centering MLP Based} & Transformer Encoder + MLP &  65.3 , + 10.7 & 150 , + 11.1 & 211 , + 11.6 & 14.1, + 6.0 \\
%         \multirow{2}{*}{} & siMLPe \cite{guo2023back} &  &  &  & - \\ \hline
%         \multirow{3}{*}{} & Diffusion Policy-CNN \cite{chi2023diffusion} &  64.1 , + 8.6 & 146 , +  8.1 & 208 , + 10.1 & 13.9 , + 4.5   \\ \hline
%         % \cline{2-6}
%         % Ours w/ Text guidance    & 93 & 12.4 & 110 & 96  &  136  & 175 &      \\ 
%         \rowcolor{green!20}
%         % \multirow{3}{*}{\centering Diffusion Based} & Ours w/ Text guidance & 57.6 , -  & 121, - 10.3 & 173, - 8.3 &  12.4 , - 7.5 \\ 

%         % \rowcolor{yellow!20}
%         \multirow{3}{*}{} & Ours   & \textbf{59} & \textbf{135} & \textbf{189} & \textbf{13.2} \\
%          \cline{2-6}
%         % Transformer Encoder + MLP & 143 & 15.3 & 167 & 148 & 203 & 256 &      \\ 

%         % \multirow{2}{*}{\centering Naïve Interpolate} & \textsc{Constant Velocity} & 149 , + 10.4\% &  101, + \% & 373 , + 95.2\%  & , + \% &  18.1 , + 35.1\%   \\ 
%     \end{tabular}}
%     \caption{Comparison of our method against prior works in visuomotor forecasting. Lower values indicate better performance.}
% \label{tab:baseline}
% \end{table*}

\renewcommand{\arraystretch}{1.1}  % Adjust row height
% \begin{table*}[h!]
% \centering
% \footnotesize 
% {\setlength{\tabcolsep}{8pt} % Adjust column spacing
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%          Methods & PA-MPJPE, \% & Head Pos., \% & Gaze Pos., \% & Hand Pos., \% & Head Rot., \%\\ \hline
%         \textsc{Constant Pose} &  68.3, +16.6 &  184, +73.6 & 193, +55.6 & 274, +45.7 & 16.7, +25.6 \\ 
%         \textsc{Constant Velocity} &  109, +84.7 & 161, +51.9 & 201, + 62.1 & 436, +132  &  18.5, +39.1 \\ 
%         Transformer Encoder + MLP &  65.3, +10.7 & 119, +12.3 & 135, +8.1 & 211, +12.2 & 13.8, +4.5 \\
%         Transformer Decoder + MLP &  60, +1.69 & 119, +12.3 & 137, +10.5 & 204, +8.5 & 14.4, +9.09 \\
%         Diffusion Policy-CNN \cite{chi2023diffusion} & 64.1, +8.6  & 112, +5.7 & 132, +6.5 & 208, +10.6 & 13.9, +5.3 \\
%         \cellcolor{green!20}\textbf{Ours} & \cellcolor{green!20}\textbf{59}  & \cellcolor{green!20}\textbf{106} & \cellcolor{green!20}\textbf{124} & \cellcolor{green!20}\textbf{188} & \cellcolor{green!20}\textbf{13.2} \\ \hline
%     \end{tabular}}
%     \caption{Quantitative comparison of our method against baselines. Lower values indicate better performance.
%     % {\color{red}TODO: add results on top 5\% hardest sample to validate simple performance. adding simple viz if have time.}
%     }
% \label{tab:baseline}
% \end{table*}


% \begin{table*}[h!]
% \centering
% \footnotesize 
% {\setlength{\tabcolsep}{8pt} % Adjust column spacing
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%          Methods & PA-MPJPE, \% & Head Pos., \% & Gaze Pos., \% & Hand Pos., \% & Head Rot., \%\\ \hline
%         \textsc{Constant Pose} &  68.3, +16.6 &  184, +73.6 & 193, +55.6 & 274, +45.7 & 16.7, +25.6 \\ 
%         \textsc{Constant Velocity} &  109, +84.7 & 161, +51.9 & 201, + 62.1 & 436, +132  &  18.5, +39.1 \\ 
%         Transformer Encoder + MLP &  65.3, +10.7 & 119, +12.3 & 135, +8.1 & 211, +12.2 & 13.8, +4.5 \\
%         Transformer Decoder + MLP &  60, +1.69 & 119, +12.3 & 137, +10.5 & 204, +8.5 & 14.4, +9.09 \\
%         Diffusion Policy-CNN \cite{chi2023diffusion} & 64.1, +8.6  & 112, +5.7 & 132, +6.5 & 208, +10.6 & 13.9, +5.3 \\
%         \cellcolor{green!20}\textbf{Ours} & \cellcolor{green!20}\textbf{59}, $\pm {\scriptstyle0.36}$ & \cellcolor{green!20}\textbf{106}, $\pm {\scriptstyle0.33}$ & \cellcolor{green!20}\textbf{124}, $\pm {\scriptstyle0.44}$ & \cellcolor{green!20}\textbf{188}, $\pm {\scriptstyle0.76}$ & \cellcolor{green!20}\textbf{13.2}, $\pm {\scriptstyle 0.08}$ \\ \hline
%     \end{tabular}}
%     \caption{Quantitative comparison of our method against baselines. Lower values indicate better performance.
%     % {\color{red}TODO: add results on top 5\% hardest sample to validate simple performance. adding simple viz if have time.}
%     }
% \label{tab:baseline}
% \end{table*}

% \renewcommand{\arraystretch}{1.1}  % Adjust row height
% \begin{table*}[h!]
% \centering
% \footnotesize 
% {\setlength{\tabcolsep}{8pt} % Adjust column spacing
%     \begin{tabular}{|c|c|c|c|c|c|c|}
%         \hline
%          Methods & PA-MPJPE, \% & Head Pos., \% & Gaze Pos., \% & Hand Pos., \% & Head Rot., \% & GRAE \\ \hline
       
%         \textsc{Constant Pose} &  68.3, +16.6 &  184,  +  73.6 & 193 , + 55.6 & 274, +45.7 & 16.7, +25.6 & \\ 
%         \textsc{Constant Velocity} &  109, +84.7 & 161, + 51.9 & 201, + 62.1 & 436, +132  &  18.5, +39.1 & 23.6 \\ 
        
%         Transformer Encoder + MLP &  65.3, +10.7 & 119,  + 12.3 & 135,  +8.1 & 211, +12.2 & 13.8, +4.5 & 20.5 \\
%         % & siMLPe \cite{guo2023back} & 61, + 3.4 & 140, + 4.5 & 189 , + 0.5 & \textbf{12.9}, -2.3 \\ 
%         % & siMLPe \cite{guo2023back} & 63, + 6.8 & 147, + 9.7 & 200 , + 5.9 & 14.5  + 9.1 \\ 
%         % \hline
%         Diffusion Policy-CNN \cite{chi2023diffusion} & 64.1, +8.6  & 112, +5.7 & 132, + 6.5 & 208, +10.6 & 13.9, +5.3 & 18.9 \\
%         % \rowcolor{green!20}
%         \cellcolor{green!20}\textbf{Ours} & \cellcolor{green!20}\textbf{59}  & \cellcolor{green!20}\textbf{106} & \cellcolor{green!20}\textbf{124} & \cellcolor{green!20}\textbf{188} & \cellcolor{green!20}\textbf{13.2} & \cellcolor{green!20}18.8 \\ \hline
%     \end{tabular}}
%     \caption{Quantitative comparison of our method against baselines. Lower values indicate better performance.
%     % {\color{red}TODO: add results on top 5\% hardest sample to validate simple performance. adding simple viz if have time.}
%     }
% \label{tab:baseline}
% \end{table*}

% {\color{blue}\subsection{Ablations}}
% \subsection{Ablations}
% \label{subsec:abla}
% To evaluate the contribution of different components in our visuomotor prediction model, we conduct an ablation study by systematically removing or modifying key elements. We compare against the following variants:

% \begin{itemize}
%     \item \textbf{w/o Gaze}: Removes gaze direction while keeping head pose intact, assessing the role of gaze as an independent cue in visuomotor coordination.
%     \item \textbf{w/o Head Rotation}: Removes head orientation as an input feature while retaining positional information, testing the impact of rotational motion cues on visuomotor representation.
%     \item \textbf{w/o Head Rotation \& Gaze}: Eliminates both head orientation and gaze direction, further evaluating the role of visual attention and rotational dynamics in predicting visuomotor states.
%     \item \textbf{w/o Head}: Excludes all head-related information (position and rotation), isolating the contribution of head pose in visuomotor coordination.
%     \item \textbf{w Last Step Arm}: Instead of using the full upper-body movement history, conditions the model only on the last observed arm configuration, evaluating the necessity of temporal context in visuomotor inference.
%     \item \textbf{w/o Egocentric Frame}: Removes egocentric visual input, leaving only kinematic information. This tests the importance of first-person visual perception in modeling visuomotor behavior.
% \end{itemize}

% \subsection{Ablations}
% \label{subsec:abla}
% To evaluate the contribution of different components in our visuomotor prediction model, we conduct an ablation study by systematically removing or modifying key elements. We compare the following variants:

% \begin{itemize}
%     \item \textbf{w/o Gaze}: Removes gaze direction while keeping head pose, assessing its role as an independent visuomotor cue.
%     \item \textbf{w/o Head Rotation}: Removes head orientation while retaining positional information, testing the impact of rotational motion cues.
%     \item \textbf{w/o Head Rotation \& Gaze}: Eliminates both head orientation and gaze, further evaluating the role of visual attention and rotational dynamics.
%     \item \textbf{w/o Head}: Excludes all head-related information, isolating its contribution to visuomotor coordination.
%     \item \textbf{w Last Step Arm}: Uses only the last observed arm configuration instead of full movement history, testing the necessity of temporal context.
%     \item \textbf{w/o Egocentric Frame}: Removes egocentric visual input, leaving only kinematics, to assess the importance of first-person perception.
% \end{itemize}

% \subsection{Ablations}
% \label{subsec:abla}
% To assess the contribution of different components in our visuomotor prediction model, we conduct an ablation study by selectively removing key inputs or excluding them from the output space. We evaluate the following variants:

% \begin{itemize}
%     \item \textbf{w/o Head Rotation}: Removes head orientation from either the input or output to test its role in visuomotor inference.
%     \item \textbf{w/o Head Rotation \& Gaze}: Removes both head orientation and gaze direction from either the input or output to assess the impact of visual attention and rotational dynamics.
%     \item \textbf{w/o Head}: Excludes all head-related information (position and rotation) from either the input or output, isolating its contribution to visuomotor coordination.
%     \item \textbf{w/o Gaze}: Removes gaze direction from either the input or output to examine its necessity as an explicit cue.
% \end{itemize}

\subsection{Ablations}
\label{subsec:abla}
To assess the contribution of different components in our visuomotor prediction model, we perform two complementary sets of ablations. The first examines how individual visuomotor signals affect prediction when removed from the input or the output, while the second evaluates the impact of high-level modality cues.

\noindent\textbf{Input–Output Ablations.}
Each ablation removes a specific signal from the model’s output space, and we additionally test whether providing that signal in the input helps compensate for its absence in the output. This design mirrors the two-row structure in Table~\ref{tab:ablation} (\bluecheck: signal available in input; {\color{red} \textbf{\xmark}}: signal removed from input).

\begin{itemize}
    \item \textbf{w/o Head Rotation}: Evaluates the role of head orientation by removing its prediction target, with or without supplying head rotation in the input.
    \item \textbf{w/o Head Rotation \& Gaze}: Tests how removing both head rotation and gaze predictions affects performance, again comparing settings with and without their input counterparts.
    \item \textbf{w/o Head}: Removes all head-related signals (position and rotation) from the output, isolating their contribution to downstream coordination.
    \item \textbf{w/o Gaze}: Removes gaze prediction to analyze how gaze supervision influences hand and head motion modeling.
\end{itemize}

\noindent\textbf{Signal Modality Ablations.}
These ablations evaluate the importance of temporal arm dynamics and egocentric perception:

\begin{itemize}
    \item \textbf{w Last Step Arm}: Replaces the full arm-motion history with only the last observed arm configuration, testing how much temporal structure is needed for accurate upper-body prediction.
    \item \textbf{w/o Egocentric Frame}: Removes egocentric visual features and relies solely on kinematic signals, assessing how first-person visual context stabilizes head–gaze coordination.
\end{itemize}


% \subsection{Ablations}
% \label{subsec:abla}
% To assess the contribution of different components in our visuomotor prediction model, we conduct two types of ablations: one focusing on specific input and output signals, and another analyzing the impact of different modalities.

% \noindent \textbf{Input-Output Ablations.} 
% We first examine the role of key visuomotor signals by selectively removing them from the input or output space:

% \begin{itemize}
%     \item \textbf{w/o Head Rotation}: Removes head rotation from the output and optionally from the input to test its necessity.
%     \item \textbf{w/o Head Rotation \& Gaze}: Removes both head rotation and gaze from the output and optionally from the input to evaluate their impact.
%     \item \textbf{w/o Head}: Removes all head-related information (position and rotation) from the output and optionally from the input.
%     \item \textbf{w/o Gaze}: Removes gaze from the output and optionally from the input to test its role.
% \end{itemize}

% \noindent \textbf{Signal Modality Ablations.} 
% We further analyze the contribution of different sensory and temporal modalities:

% \begin{itemize}
%     \item \textbf{w Last Step Arm}: Uses only the last observed arm configuration instead of the full motion history to evaluate the importance of temporal context.
%     \item \textbf{w/o Egocentric Frame}: Removes egocentric visual input, leaving only kinematic information, to assess the role of first-person vision in visuomotor prediction.
% \end{itemize}

\begin{table*}[htbp]
\centering
\footnotesize 
{\setlength{\tabcolsep}{8pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1} % Default value: 1
    \begin{tabular}{ccccccc}
        \toprule
        % \multicolumn{1}{c|}{\multirow{2}{*}{}} &\multicolumn{2}{c|}{Head Pose} &\multicolumn{1}{c|}{Gaze Pose} &\multicolumn{3}{c|}{Arm Pose} & \multicolumn{1}{|c}{}\\ 
        % \cline{2-8}
        % \hline
         \textbf{Ablations} & \textbf{Input} & \textbf{Head Pos., \%} & \textbf{Gaze Pos., \%} & \textbf{Hand Pos., \%} & \textbf{Head Rot., \%} & \textbf{PA-MPJPE, \%} \\ \midrule
        \rowcolor{green!20}\textbf{}
        Complete Visuomotor  & - & \textbf{106} & \textbf{124} & \textbf{188} & \textbf{13.2} & \textbf{59}\\ \hline
        % \multicolumn{7}{c}{\textbf{Input-Output Ablations}} \\ \hline
        \multicolumn{7}{c}{\cellcolor{yellow!20}\textbf{Input-Output Ablations}} \\ \hline
        Head Rotation  & \bluecheck & 108, + 1.9 & 126, + 1.6 & 188, + 0.0 & {\color{red} \textbf{\xmark}} & \multirow{8}{*}{\centering \parbox{3cm}{\centering \textit{Metric unavailable due to incomplete output space}}} \\
        Head Rotation  & {\color{red} \textbf{\xmark}}  & 111, + 4.7 & 130, + 4.8 & 195, + 3.7 & {\color{red} \textbf{\xmark}} &  \\ \cline{1-6}
        Head Rotation \& Gaze  & \bluecheck & 109, + 2.8 &  {\color{red} \textbf{\xmark}}  & 190, + 1.1 & {\color{red} \textbf{\xmark}} &  \\
        Head Rotation \& Gaze  & {\color{red} \textbf{\xmark}} & 112, + 5.7 & {\color{red} \textbf{\xmark}} & 196, + 4.3 & {\color{red} \textbf{\xmark}} & \\ \cline{1-6}
        Head  & \bluecheck & {\color{red} \textbf{\xmark}}  & 127, + 2.4 & 190, + 1.1 & {\color{red} \textbf{\xmark}} &  \\
        Head  & {\color{red} \textbf{\xmark}} & {\color{red} \textbf{\xmark}} & 132, + 6.5 & 194, + 3.2 & {\color{red} \textbf{\xmark}} &  \\ \cline{1-6}
        Gaze  & \bluecheck & 109, + 2.8  & {\color{red} \textbf{\xmark}} & 190, +1.1 & 13.4, +1.5 &  \\ 
        Gaze  & {\color{red} \textbf{\xmark}} & 111, + 4.7 & {\color{red} \textbf{\xmark}}  & 194, + 3.2 & 13.9, + 4.5 &  \\ 
        \hline 
        % \multicolumn{7}{c}{\textbf{Signal Modality Ablations}} \\ \hline
        \multicolumn{7}{c}{\cellcolor{yellow!20}\textbf{Signal Modality Ablations}} \\ \hline
        % Modality Ablations & &  &  Head Pos. , \% & Gaze Pos. , \% & Hand Pos. , \% & Head Rot. , \% & \% PA-MPJPE, \% \\ \hline
        % Full Visuomotor & & & \textbf{59} & \textbf{106} & \textbf{124} & \textbf{188} & \textbf{13.2} \\ 
        w Last Step Arm & - & 113, + 6.6 & 141, + 5.2 & 199, + 5.9 & 13.7 , + 3.8  & 61, + 3.4 \\
        w/o Egocentric Frames & - & 111, + 4.7 & 130, + 4.8 & 193, + 2.7 & 14.1 , + 6.0 &  60, + 1.7 \\
        \bottomrule
    \end{tabular}}
    % \vspace{-6pt}
    % \caption{\textbf{Ablation Study on Input Configuration and Signal Modalities.} The table presents two sets of ablations: \textit{(1) Input-Output Ablations}, which evaluate the impact of removing specific kinematic inputs (head rotation, head position, gaze, and upper-body joints) on prediction accuracy, and \textit{(2) Signal Modality Ablations}, which assess the effect of removing higher-level input signals such as the last-step arm pose and egocentric frames. The \textit{Complete Visuomotor} row represents the full model, achieving the lowest error across all metrics.}

    % \caption{\textbf{Ablation Study on Input Configuration and Signal Modalities} We report two types of ablations: \textit{(1) Input–Output Ablations}, which remove a modality from the output while optionally keeping it in the input. This mismatch is intentional and quantifies how strongly other components depend on the removed signal. \textit{(2) Signal Modality Ablations}, which remove higher-level signals such as the last-step arm pose or egocentric frame. Rows with incomplete output space do not support PA-MPJPE. We omit the setting “X excluded in input but included in output”, as predicting a modality whose reference frame depends on missing inputs (e.g., gaze without head orientation) is not physically meaningful. The \textit{Complete Visuomotor} row represents the full model, achieving the lowest error across all metrics.}
    \caption{\textbf{Ablation Study.} We evaluate two categories of ablations: \textit{(1) Input–Output ablations}, which remove a signal from the output and optionally from the input (\bluecheck present; {\color{red}\textbf{\xmark}} absent), and \textit{(2) Signal Modality ablations}, which remove higher-level cues such as previous step arm pose or egocentric frames. PA-MPJPE is omitted for settings with an incomplete output space as the metric requires a full joint set. The \textit{Complete Visuomotor} row represents the full model and achieves the best performance (lowest error) across all metrics.}
    % Settings with incomplete output space do not report PA-MPJPE. The \textit{Complete Visuomotor} row corresponds to the full model and yields the lowest error across all metrics.}

    \vspace{-6pt}
    % \vspace{-12pt}

    % \caption{Ablation study analyzing the impact of different input modalities on model performance.}
\label{tab:ablation}
\end{table*}

% To evaluate the model’s ability to maintain stable visuomotor predictions under uncertain perception conditions, we conduct a robustness analysis where specific input modalities are randomly either preserved or replaced with noise with a probability of 50\% at inference time. This process aims to simulate real-world scenarios where certain visuomotor cues may be partially observable, noisy, or occluded due to sensor limitations or environmental factors. Specifically, we examine the following cases:
% \begin{itemize}
%     \item \textbf{Stochastic Head Pose Dropout}: Head pose is randomly kept or replaced with noise, requiring the model to infer head dynamics.
%     \item \textbf{Stochastic Gaze Dropout}: Gaze direction is randomly available or noisy, challenging the model to estimate attention patterns.
%     \item \textbf{Stochastic Arm Motion Dropout}: Upper-body joints are randomly kept or noised, testing the model’s ability to predict arm motion.
% \end{itemize}

\subsection{Quantitative Results}
\label{subsec:quanti}
Tables~\ref{tab:baseline} and~\ref{tab:ablation} summarize our results: baseline comparisons, ablation studies on different input modalities, and per-class prediction performance, respectively. The best results are highlighted in bold, and lower values across all metrics indicate better performance (Sec.~\ref{subsec:dataset}).

% \noindent \textbf{Comparison with Baseline Methods.}
% Table~\ref{tab:baseline} compares our model with two naïve forecasting heuristics and three learning-based predictors. We first examine naïve interpolation baselines, \textit{Constant Pose} and \textit{Constant Velocity}, which assume either no future motion or simple linear extrapolation. As expected, these methods are insufficient for modeling complex visuomotor behavior: Constant Pose yields a PA-MPJPE of 68 and a hand error of 274, while Constant Velocity produces a PA-MPJPE of 109 and a hand error of 436.

% Learning-based approaches achieve substantially lower errors, highlighting the importance of temporal modeling and multimodal conditioning. The \textit{Transformer Encoder + MLP} baseline performs reasonably well, reflecting the benefit of sequence modeling with visual features. We further include a \textit{Transformer Decoder} model, which generates future states using learned queries and cross-attention, and an \textit{Autoregressive Head} that predicts motion step-by-step on top of the encoder baseline. The autoregressive variant performs noticeably worse due to error accumulation and its limited temporal receptive field.

\noindent \textbf{Comparison with Baseline Methods.}
Table~\ref{tab:baseline} compares our method with two naïve interpolation heuristics and three learning-based predictors. As expected, \textit{Constant Pose} and \textit{Constant Velocity} fail to capture complex visuomotor dynamics, yielding large PA-MPJPE and hand errors (68/274 and 109/436, respectively).

Learning-based models perform substantially better. The \textit{Transformer Encoder + MLP} baseline benefits from temporal sequence modeling and visual features. We also evaluate a \textit{Transformer Decoder} variant that predicts future states from learned queries via cross-attention, and an \textit{Autoregressive Head} that predicts each timestep sequentially. The autoregressive model performs worse due to error accumulation across timesteps.

Our model achieves a PA-MPJPE of 59, improving upon the strongest baseline, \textit{Diffusion Policy–CNN}, by 7.8\%, and upon the \textit{Transformer Encoder + MLP} baseline by 9.2\%. Similar gains appear across head, gaze, and hand position metrics; for example, our model reduces head and gaze position error by 5.4\% and 6.1\% relative to \textit{Diffusion Policy–CNN}. These improvements indicate that our approach yields more accurate visuomotor forecasts while maintaining coherent multimodal coordination.

The largest performance gain is observed in hand prediction, the most challenging component of the visuomotor state. This suggests that our structured representation effectively captures head–eye–hand dependencies and supports fine-grained motion prediction. In terms of orientation, our model achieves an average head rotation error of 13.2 degrees, outperforming \textit{Diffusion Policy–CNN} by 5.0\%. The consistent improvements across both rotational and translational metrics demonstrate that our method learns a unified visuomotor representation capable of handling diverse motion modalities within a single framework.

\noindent \textbf{Ablation Study.}  
Table~\ref{tab:ablation} evaluates the impact of removing different input components on visuomotor prediction. The \textit{Complete Visuomotor} setting (row 0) includes all available inputs (head pose, gaze, and upper-body joints), while the ablations systematically remove each to examine its role.  

Removing head rotation (row 2) increases head position error from 106 to 111, while additionally removing gaze input (row 4) further degrades performance to 112. Gaze position error rises from 124 to 130, and hand position error increases from 188 to 196, highlighting the importance of head and gaze signals for accurate motion prediction. When all head-related inputs are removed (row 6), gaze error increases from 124 to 132, and hand error from 188 to 194, indicating that head motion affects overall visuomotor coordination. The absence of gaze input (row 8) also increases head rotation error from 13.2 to 13.9, confirming its role in stabilizing head orientation.  

The lower section of Table~\ref{tab:ablation} examines high-level signal ablations. Preserving only the last-step arm pose (\textit{w/ Last Step Arm}) increases head, gaze, and hand errors by 6.6\%, 5.2\%, and 5.9\%, respectively, suggesting that a single arm pose lacks sufficient temporal context for predicting upper-body motion. Removing egocentric vision (\textit{w/o Egocentric Frames}) leads to 4.7\% higher head position error and a 6\% increase in head rotation error, reinforcing the role of visual context in stabilizing head and gaze coordination. Interestingly, gaze error increases from 124 to 130, suggesting a shift toward kinematic reliance for gaze estimation.  

These results confirm that multimodal integration enhances predictive visuomotor coordination: temporal kinematic history improves hand predictions, while egocentric vision stabilizes head and gaze alignment.

\definecolor{gtcolor}{RGB}{50,253,212}

\begin{figure*}[t]
  \centering
   \includegraphics[width=1.0\linewidth]{figs/qualitative.png}
    \vspace{-24pt}
    % \caption{Visualization of predicted visuomotor coordination across diverse real-world scenes. Each row corresponds to a different scene, while columns illustrate the temporal evolution of visuomotor coordination. The {\color{yellow}{\textbf{first column}}} represents the observed states, while subsequent columns show predictions from time step 2 to 10. {\color{magenta}{\textbf{Predicted poses}}} and {\color{cyan}{\textbf{ground truth poses}}} are overlaid for interoperability. View in color for best results. }
    \caption{\textbf{Visualization of predicted visuomotor coordination across diverse real-world scenes.} Each row corresponds to a different scene, while columns illustrate the temporal evolution of visuomotor coordination. The {\color{yellow}{\textbf{first column}}} represents the observed states, while subsequent columns display predictions from time step 2 to 10. {\color{magenta}{\textbf{Predicted poses}}} and {\color{gtcolor}{\textbf{ground truth poses}}} are overlaid for interpretability. View in color for best results. Note that the background point cloud is visualized only for context and is not used as input to the model.}
   \label{fig:qualitative}
   \vspace{-12pt}

\end{figure*}

\subsection{Qualitative Results}  
\label{subsec:quali}

Figure~\ref{fig:qualitative} illustrates the predicted visuomotor coordination across diverse real-world scenes. 
The model accurately captures the coupled evolution of head, gaze, and upper-body motion, producing smooth and temporally consistent predictions. 
As shown in Rows (a)-(d), it successfully anticipates head and gaze shifts, even under scene constraints, demonstrating its ability to infer visuomotor intent from prior observations.

Failure cases arise in highly dynamic scenarios where abrupt movements introduce uncertainty that is difficult to resolve from preceding frames alone. 
Row (e) shows a representative example: as a basketball abruptly changes direction, the ground-truth motion involves a rapid rightward shift that only becomes evident at the last input frame. 
Our model predicts a more typical catching motion, resulting in a temporal lag relative to the true visuomotor adjustment. 
These errors highlight the sensitivity of visuomotor coordination to subtle, transient cues that may not be fully captured by standard kinematic conditioning. 
Despite these challenges, the model remains robust across most activities, reinforcing the value of multimodal fusion in learning coordinated visuomotor behavior. 
Future extensions may incorporate explicit contact reasoning or environmental cues to improve performance in fast, event-driven tasks. 
Additional video examples are included in the supplementary for more comprehensive qualitative analysis.


% Figure~\ref{fig:qualitative} illustrates the predicted visuomotor coordination across diverse real-world scenes. The model effectively captures head, gaze, and upper-body dynamics, maintaining smooth and temporally consistent motion. As shown in Rows (a)-(d), it successfully anticipates head and gaze shifts, even under scene constraints, demonstrating its ability to infer visuomotor intent from prior observations.

% However, failure cases occur in scenarios with rapid, unexpected movements or occlusions, where subtle cues are insufficient for precise coordination. While our model still produces reasonable predictions, it may misalign with the ground truth. Row (e) presents a typical failure case: as the basketball bounces quickly—a nuance observable only in the last frame of the egocentric input—the person rapidly shifts their body rightward to catch it. In contrast, our prediction assumes a standard catching motion, failing to adapt to the sudden trajectory change. Despite these challenges, overall prediction quality remains strong, reinforcing the effectiveness of multimodal integration in learning visuomotor coordination. Future improvements could involve incorporating explicit contact modeling or leveraging environment-aware reasoning to enhance robustness in highly dynamic tasks. For a more comprehensive demonstration, we provide video examples in the supplementary.



==> sec/5_conclusion.tex <==
\section{Conclusion}  
We introduce a forecasting-based task for human visuomotor modeling, aiming to predict future head pose, gaze, and upper-body motion from egocentric visual and kinematic observations. Central to our approach is the Visuomotor Coordination Representation, which captures structured temporal dependencies across multimodal signals. We build upon diffusion-based motion modeling by integrating egocentric visual context with kinematic sequences, enabling temporally coherent and accurate visuomotor prediction. Evaluations on the large-scale EgoExo4D dataset demonstrate strong generalization across a wide range of real-world activities. Our experiments highlight the importance of multimodal integration for modeling visuomotor coordination. The resulting framework advances structured human motion representation with relevance to robotics, human–computer interaction, and assistive technologies.
% We introduced a forecasting-based task for human visuomotor modeling, where the goal is to predict future head pose, gaze, and upper-body motion from egocentric visual and kinematic observations. To achieve this, we proposed the \textit{Visuomotor Coordination Representation}, which learns structured temporal dependencies across multimodal signals. We further extended a diffusion-based motion modeling framework integrating egocentric vision and kinematic sequences, enabling temporally coherent and accurate visuomotor predictions. Our approach was evaluated on the challenging large-scale EgoExo4D dataset, demonstrating strong generalization across diverse real-world activities. Through extensive experiments, we showed that multimodal integration plays a crucial role in visuomotor modeling. Our results provide insights into structured human motion representation, with applications in robotics, human-computer interaction, and assistive technologies.  
\newpage
\noindent \textbf{Acknowledgements.} This work was supported in part by the Health Care Engineering Systems Center at UIUC. We thank Ruocheng Wang for valuable discussion and feedback on the paper. 



\begin{table*}[htbp]
\centering
\footnotesize 
{\setlength{\tabcolsep}{8pt} % Default value: 6pt
    \begin{tabular}{cccccc}
        \toprule
         \textbf{Ablations} & \textbf{Head Pos., \%} & \textbf{Gaze Pos., \%} & \textbf{Hand Pos., \%} & \textbf{Head Rot., \%} & \textbf{PA-MPJPE, \%} \\ \midrule
        \rowcolor{green!20}\textbf{}
        Full Model  & \textbf{106} & \textbf{124} & \textbf{188} & \textbf{13.2} & \textbf{59}\\ \hline
        \multicolumn{6}{c}{\cellcolor{yellow!20}\textbf{Input-Output Ablations}} \\ \hline
        % Head Rotation  & \bluecheck & 108, + 1.9 & 126, + 1.6 & 188, + 0.0 & {\color{red} \textbf{\xmark}} & \multirow{8}{*}{\centering \parbox{3cm}{\centering \textit{Metric unavailable due to incomplete output space}}} \\
        % Head Rotation  & {\color{red} \textbf{\xmark}}  & 111, + 4.7 & 130, + 4.8 & 195, + 3.7 & {\color{red} \textbf{\xmark}} &  \\ \cline{1-6}
        % Head Rotation \& Gaze  & \bluecheck & 109, + 2.8 &  {\color{red} \textbf{\xmark}}  & 190, + 1.1 & {\color{red} \textbf{\xmark}} &  \\
        w/o Head Rotation \& Gaze  & 112, + 5.7 & {\color{red} \textbf{\xmark}} & 196, + 4.3 & {\color{red} \textbf{\xmark}} & -- \\ \cline{1-6}
        % Head  & \bluecheck & {\color{red} \textbf{\xmark}}  & 127, + 2.4 & 190, + 1.1 & {\color{red} \textbf{\xmark}} &  \\
        % Head  & {\color{red} \textbf{\xmark}} & {\color{red} \textbf{\xmark}} & 132, + 6.5 & 194, + 3.2 & {\color{red} \textbf{\xmark}} &  \\ \cline{1-6}
        % Gaze  & \bluecheck & 109, + 2.8  & {\color{red} \textbf{\xmark}} & 190, +1.1 & 13.4, +1.5 &  \\ 
        % Gaze  & {\color{red} \textbf{\xmark}} & 111, + 4.7 & {\color{red} \textbf{\xmark}}  & 194, + 3.2 & 13.9, + 4.5 &  \\ 
        \hline 
        \multicolumn{6}{c}{\cellcolor{yellow!20}\textbf{Signal Modality Ablations}} \\ \hline
        w Last Step Arm & 113, + 6.6 & 141, + 5.2 & 199, + 5.9 & 13.7 , + 3.8  & 61, + 3.4 \\
        w/o Egocentric Frames & 111, + 4.7 & 130, + 4.8 & 193, + 2.7 & 14.1 , + 6.0 &  60, + 1.7 \\
        \bottomrule
    \end{tabular}}
    \caption{\textbf{Ablation Study.} We evaluate two categories of ablations: \textit{(1) Input–Output ablations}, which remove a signal from the output and optionally from the input (\bluecheck present; {\color{red}\textbf{\xmark}} absent), and \textit{(2) Signal Modality ablations}, which remove higher-level cues such as previous step arm pose or egocentric frames. PA-MPJPE is omitted for settings with an incomplete output space as the metric requires a full joint set. The \textit{Complete Visuomotor} row represents the full model and achieves the best performance (lowest error) across all metrics.}
    \vspace{-6pt}
\label{tab:ablation}
\end{table*}
